Low-Depth Parallel Algorithms for the Binary-Forking Model without Atomics

The binary-forking model is a parallel computation model, formally defined by Blelloch et al. very recently, in which a thread can fork a concurrent child thread, recursively and asynchronously. The model incurs a cost of $\Theta(\log n)$ to spawn or synchronize $n$ tasks or threads. The binary-forking model realistically captures the performance of parallel algorithms implemented using modern multithreaded programming languages on multicore shared-memory machines. In contrast, the widely studied theoretical PRAM model does not consider the cost of spawning and synchronizing threads, and as a result, algorithms achieving optimal performance bounds in the PRAM model may not be optimal in the binary-forking model. Often, algorithms need to be redesigned to achieve optimal performance bounds in the binary-forking model and the non-constant synchronization cost makes the task challenging. Though the binary-forking model allows the use of atomic {\em test-and-set} (TS) instructions to reduce some synchronization overhead, assuming the availability of such instructions puts a stronger requirement on the hardware and may limit the portability of the algorithms using them. In this paper, we avoid the use of locks and atomic instructions in our algorithms except possibly inside the join operation which is implemented by the runtime system. In this paper, we design efficient parallel algorithms in the binary-forking model without atomics for three fundamental problems: Strassen's (and Strassen-like) matrix multiplication (MM), comparison-based sorting, and the Fast Fourier Transform (FFT). All our results improve over known results for the corresponding problem in the binary-forking model both with and without atomics.

==> algorithms.tex <==
\section{Hybrid Algorithms}
\label{sec:algorithms}

In this section, we develop hybrid divide-and-conquer algorithms for three types of problems: dynamic programming, tensor product and spatial tree based computation like Barnes-hut algorithm. In dynamic programming we have developed hybrid algorithm for multi-instance Viterbi algorithm, Floyd-Warshall's all-pairs shortest path, and protein accordion folding.

\subsection{\textbf{Dynamic Programming}}
In this subsection, we prove that if a dynamic programming algorithm follows some property, there exist space-parallelism tradeoff. 
\begin{theorem}[\highlighttitle{Existence Theorem}]
	\label{thm:exist}
	Let $\m{F}_1, \m{F}_2, \ldots, \m{F}_m$ be the $m$ functions of the in-place recursive dynamic programming algorithm. Let the span of the functions be computed as follows:

\begin{align*}
T_{\m{F}_i} (n) &= \begin{cases} 1 &\mbox{if } n = 1, \\ 
\sum_{j = i}^{m} a_{ij} T_{\m{F}_j} \left( n/2 \right) + \Th{1}  & \mbox{otherwise}  \end{cases}
\end{align*}



where, $T_{\m{F}_i}(n)$ is the span of $\m{F}_i(n)$ and $a_{ij}$ is the number of parallel steps in which the function $\m{F}_i$ calls $\m{F}_j$. Let $k_{i}$ denotes the number of times, function $\m{F}_{i}$ calls itself. A function $\m{F}_i$ is called dominating if $\forall j\in [1\ldots m]: k_i\ge k_j$. Suppose the function $\m{F}_m$ be like matrix-multiplication reading from submatrices, it does not write to and also that $\m{F}_m$ is dominating. Also, let $maximum =  \textsc{max}{\{a_{11}, a_{22}, \ldots, a_{mm}\}}$.

If $maximum = 2$, then there exist not-in-place and hybrid algorithms to asymptotically increase parallelism.
\end{theorem}

\begin{proof}

Let $P = \m{F}_{r_1},\m{F}_{r_2}, \ldots, \m{F}_{|P|}$ be a path in the recursion tree of the root $(=\m{F}_{r_1} = \m{F}_{1})$ to a node corresponding to $\m{F}_{m} (= \m{F}_{|P|})$. Let $q$ out of these $|P|$ functions call themselves in $(maximum = 2)$ parallel steps and $q$ is maximized over all possible paths in the recursion tree. Then the span of the in-place algorithm is
\begin{equation}
T_{\m{F}_1} (n) = \Th{n \log^{q - 1} n} \qquad (\text{in-place algorithm})
\end{equation}
which is found by recursively applying the master theorem from the leaf of the recursion tree to the root.


We know that $\m{F}_m$ is matrix multiplication algorithm (or any matrix-multiplication-like kernel) and there is a not-in-place algorithm for it whose span recurrence is 

\begin{equation}
T_{\m{F}_m} (n) = T_{\m{F}_m} \left( \frac{n}{2} \right) + \Th{1} \qquad \text{if n > 1.}
\end{equation}

It is important to note that replacing the in-place MM-like algorithm $\m{F}_m$ with a not-in-place algorithm, the value of $q$ will be decremented by 1. This gives rise to the not-in-place algorithm with span

\begin{align*}
T_{\m{F}_1} (n) &= \begin{cases} \Th{\log n} &\mbox{if } q = 1, \\ 
	\Th{n \log^{q - 1} n}  & \mbox{if } q > 1. \end{cases}
\end{align*}


This implies that there is a not-in-place algorithm with asymptotic decrease in span (or asymptotic increase in parallelism). Hence, there is a hybrid algorithm with asymptotic increase in parallelism.

\end{proof}
In the following three subsections, we show that three instances of dynamic programming problem such as Multi-instance Viterbi algorithm, Floyd-Warshall algorithm and Protein accordion folding obey Existence Theorem presented in Theorem \ref{thm:exist} and there is a space-parallelism tradeoff. 

\subsubsection{Multi-instance Viterbi algorithm}
The Viterbi algorithm (VA) \cite{Viterbi1967, Viterbi1971} proposed by Andrew J. Viterbi is a DP algorithm that finds the most probable sequence of hidden states from a given sequence of observed events. The algorithm is used in decoding method for convolutional codes in noisy communication channels, Qualcomm's CDMA technology \cite{KleinPaViWeWh1991, KandWi1998}, and part-of-speech tagging \cite{CuttingKuPeSi1992, TaylorBl1998}.

The Viterbi algorithm is described as follows. We are given an observation space $O = \{ o_1, o_2, \ldots, o_m \}$, state space $S = \{ s_1, s_2, \ldots, s_n \}$, observations $Y = \{ y_1, y_2, \ldots, y_t \}$, transition matrix $A$ of size $n \times n$, where $A[i, j]$ is the transition probability of transiting from $s_i$ to $s_j$, emission matrix $B$ of size $n \times m$, where $B[i, j]$ is the probability of observing $o_j$ at $s_i$, and initial probability vector (or initial solution vector) $I$, where $I[i]$ is the probability that $x_i = s_i$. Let $X = \{x_1, x_2, \ldots, x_t\}$ be a sequence of hidden states that generates $Y = \{ y_1, y_2, \ldots, y_t \}$. Then the matrices $P$ and $P^{\prime}$ of size $n \times t$, where $P[i, j]$ is the probability of the most likely path of getting to state $s_i$ at observation $o_j$ and $P^{\prime}[i, j]$ stores the hidden state of the most likely path (i.e., Viterbi path) are computed as follows. Here, we compute only matrix $P$ as the computation of $P$ dominates computation of $P^{\prime}$.
\vspace{-0.1cm}
{\small
	\begin{align*}
	P[i, j] &= \left\{ \begin{array}{ll}
	I[i] \cdot B[i, y_1] & \textrm{if $j = 1$,}\\
	\underset{k \in [1, n]}{\textrm{max}} (P[k, j-1] \cdot A[k, i] \cdot B[i, y_j])
	& \textrm{if $j > 1$.}
	\end{array} \right.\\
	P^{\prime}[i, j] &= \left\{ \begin{array}{ll}
	0 & \textrm{if $j = 1$,}\\
	\textrm{arg} \underset{k \in [1, n]}{\textrm{max}} (P[k, j-1] \cdot A[k, i] \cdot B[i, y_j])
	& \textrm{if $j > 1$.}
	\end{array} \right.
	\label{eq:viterbi}
	\end{align*}
}

\begin{figure}[!ht]
	\centering
	\begin{minipage}{0.47\textwidth}
		\begin{mycolorbox}{\textsc{Multi-Instance-Viterbi}{}$(P_1, P_2, \ldots, P_n, A, B, t)$}
			\begin{minipage}{0.99\textwidth}
				{\tiny
					\algotopspace{}
					\noindent
					\begin{enumerate}
						\setlength{\itemindent}{-2em}
						
						\vsitem \xfor $j \leftarrow 2$ \xto $t$ \xdo
						\vsitem \T $X \leftarrow [P_1[..,j], P_2[..,j], \ldots, P_n[..,j]]$
						\vsitem \T $U \leftarrow [P_1[..,j-1], P_2[..,j-1], \ldots, P_n[..,j-1]]$
						\vsitem \T $V \leftarrow A$
						\vsitem \T $W \leftarrow [B[.., y_{1j}], B[.., y_{2j}], \ldots, B[.., y_{nj}]]$
						\vsitem \T $\m{A}_{VA}(X, U, V, W)$
						
						\algobottomspace{}
					\end{enumerate}
				}
			\end{minipage}
		\end{mycolorbox}
		\vspace{0.1cm}
		\begin{mycolorbox}{$\m{A}_{VA}(X_{n \times n}, U_{n \times n}, V_{n \times n}, W_{n \times n})$}
			\begin{minipage}{0.99\textwidth}
				{\tiny
					\algotopspace{}
					\noindent
					\begin{enumerate}
						\setlength{\itemindent}{-2em}
						
						\vsitem \xif $X$ and $V$ are small matrices \xthen $\m{A}_{loop-VA}(X, U, V, W)$
						
						\vsitem \xelse
						\vsitem \T \xpar $\m{A}_{VA}(X_{11},U_{11}, V_{11}, W_{11})$, $\m{A}_{VA}(X_{12}, U_{12}, V_{11}, W_{12})$,
						\vsitem[] \xblankpar $\m{A}_{VA}(X_{21}, U_{11}, V_{12}, W_{21})$, $\m{A}_{VA}(X_{22}, U_{12}, V_{12}, W_{22})$
						
						\vsitem \T \xpar $\m{A}_{VA}(X_{11},U_{21}, V_{21}, W_{11})$, $\m{A}_{VA}(X_{12}, U_{22}, V_{21}, W_{12})$,
						\vsitem[] \xblankpar $\m{A}_{VA}(X_{21}, U_{21}, V_{22}, W_{21})$, $\m{A}_{VA}(X_{22}, U_{22}, V_{22}, W_{22})$
						
						\algobottomspace{}
					\end{enumerate}
				}
			\end{minipage}
		\end{mycolorbox}
		\vspace{-0.1cm}
	\end{minipage}
	\caption{Cache-efficient parallel recursive divide-and-conquer-based Viterbi algorithm. The matrix $U$ is 
		constructed by combining column $j-1$ of each of the $q$ problem instances $P_1, \ldots, P_n$. Note that we need not store the entire matrices $P_1, \ldots, P_n$.}
	\label{fig:viterbi}
	\vspace{-0.2cm}
\end{figure}

\begin{theorem}[\highlighttitle{Hybrid VA}]
	\label{thm:hybridva}
	The hybrid multi-instance Viterbi algorithm, assuming a tall cache, has a complexity of $T_1(n) = \Th{n^3t}$, $Q_1^{RELEASE}(n) = \Oh{n^3t/(B\sqrt{M})}$, \\ $Q_1^{RETAIN}(n) = \Oh{n^3t/(B\sqrt{M}) + 2^k n^2 t / B + 4^k n t}$,\\ $T_{\infty}(n)=\Oh{kt(2\log n - k)+nt/2^k}$, and $S(n) = \Oh{2^k n^2}$.
\end{theorem}

\subsubsection{Floyd-Warshall's all-pairs shortest path}
Floyd-Warshall's algorithm (FW) for finding all-pairs shortest path (APSP) \cite{Floyd1962} belongs 
to a class of dynamic programs that compute paths over a closed semiring in a directed graph \cite{Ullman1974}. A recursive divide-and-conquer algorithm for FW is given in \cite{ChowdhuryRa2010}. The algorithm has four functions $\m{A}, \m{B}, \m{C}$, and $\m{D}$. Due to space constraints, we do not give the algorithm here. The $\m{D}$ function in the algorithm is matrix-multiplication-like and dominates the total work complexity. Hence, by simply modifying the $\m{D}$ function to use extra space, we end up with not-in-place FW algorithm. 

\begin{figure}[!ht]
	{\scriptsize
		\begin{center}
			\vspace{-0.1cm}
			\begin{minipage}{0.48\textwidth}
				\begin{mycolorbox}{\F{\m{A}^{\phantom{2D}}}{FW}$( X,X,X )$}
					\begin{minipage}{0.99\textwidth}
						{\tiny
							\algotopspace{}
							\noindent
							\begin{enumerate}
								\setlength{\itemindent}{-2em}
								
								\vsitem \xif $X$ is a small matrix \xthen \L{\m{A}^{\phantom{2D}}}{FW}$( X,X,X )$
								
								\vsitem \xelse
								
								\vsitem \T \F{\m{A}^{\phantom{2D}}}{FW}$( X_{11},X_{11},X_{11} )$
								
								\vsitem \T \xpar \F{\m{B}^{\phantom{2D}}}{FW}$( X_{12},X_{11}X_{12} )$,~\F{\m{C}^{\phantom{2D}}}{FW}$( X_{21},X_{21},X_{11} )$
								
								\vsitem \T \F{\m{D}^{\phantom{2D}}}{FW}$( X_{22},X_{21},X_{12} )$
								
								\vsitem \T \F{\m{A}^{\phantom{2D}}}{FW}$( X_{22},X_{22},X_{22} )$
								
								\vsitem \T \xpar \F{\m{B}^{\phantom{2D}}}{FW}$( X_{21},X_{22},X_{21} )$,~\F{\m{C}^{\phantom{2D}}}{FW}$( X_{12},X_{12},X_{22} )$
								
								\vsitem \T \F{\m{D}^{\phantom{2D}}}{FW}$( X_{11},X_{12},X_{21} )$
								
								\algobottomspace{}
							\end{enumerate}
							%\medskip\noindent{\func{\F{A}{FW} Ends}}
						}
					\end{minipage}
				\end{mycolorbox}
				\vspace{0.1cm}
				\begin{mycolorbox}{\F{\m{B}^{\phantom{2D}}}{FW}$( X,U,X )$}
					\begin{minipage}{0.99\textwidth}
						{\tiny
							\algotopspace{}
							\noindent
							\begin{enumerate}
								\setlength{\itemindent}{-2em}
								
								\vsitem \xif $X$ is a small matrix \xthen \L{\m{B}^{\phantom{2D}}}{FW}$( X,U,X )$
								
								\vsitem \xelse
								
								\vsitem \T \xpar \F{\m{B}^{\phantom{2D}}}{FW}$( X_{11},U_{11},X_{11} )$,~\F{\m{B}^{\phantom{2D}}}{FW}$( X_{12},U_{11},X_{12} )$
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{21},U_{21},X_{11} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{22},U_{21},X_{12} )$
								
								\vsitem \T \xpar \F{\m{B}^{\phantom{2D}}}{FW}$( X_{21},U_{22},X_{21} )$,~\F{\m{B}^{\phantom{2D}}}{FW}$( X_{22},U_{22},X_{22} )$
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{11},U_{12},X_{21} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{12},U_{12},X_{22} )$
								
								\algobottomspace{}
							\end{enumerate}
							%\medskip\noindent{\func{\F{B}{FW} Ends}}
						}
					\end{minipage}
				\end{mycolorbox}
				\vspace{0.1cm}
				\begin{mycolorbox}{\F{\m{C}^{\phantom{2D}}}{FW}$( X,X,V )$}
					\begin{minipage}{0.99\textwidth}
						{\tiny
							\algotopspace{}
							\noindent
							\begin{enumerate}
								\setlength{\itemindent}{-2em}
								
								\vsitem \xif $X$ is a small matrix \xthen \L{\m{C}^{\phantom{2D}}}{FW}$( X,X,V )$
								
								\vsitem \xelse
								
								\vsitem \T \xpar \F{\m{C}^{\phantom{2D}}}{FW}$( X_{11},X_{11},V_{11} )$,~\F{\m{C}^{\phantom{2D}}}{FW}$( X_{21},X_{21},V_{11} )$
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{12},X_{11},V_{12} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{22},X_{21},V_{12} )$
								
								\vsitem \T \xpar \F{\m{C}^{\phantom{2D}}}{FW}$( X_{12},X_{12},V_{22} )$,~\F{\m{C}^{\phantom{2D}}}{FW}$( X_{22},X_{22},V_{22} )$
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{11},X_{12},V_{21} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{21},X_{22},V_{12} )$
								
								\algobottomspace{}
							\end{enumerate}
							%\medskip\noindent{\func{\F{C}{FW} Ends}}
						}
					\end{minipage}
				\end{mycolorbox}
				\vspace{0.1cm}
				\begin{mycolorbox}{\F{\m{D}^{\phantom{2D}}}{FW}$(X, U, V )$}
					\begin{minipage}{0.99\textwidth}
						{\tiny
							\algotopspace{}
							\noindent
							\begin{enumerate}
								\setlength{\itemindent}{-2em}
								
								% \vsitem \xif $X$ is a $1 \times 1$ matrix \xthen $X \leftarrow \min\left\{ X, U + V \right\}$
								
								\vsitem \xif $X$ is a small matrix \xthen \L{\m{D}^{\phantom{2D}}}{FW}$( X,U,V )$
								
								\vsitem \xelse
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{11}, U_{11}, V_{11} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{12}, U_{11}, V_{12} )$,
								
								\vsitem[] \xblankpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{21},U_{21}, V_{11} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{22}, U_{21}, V_{12} )$
								
								\vsitem \T \xpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{11}, U_{12}, V_{21} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{12}, U_{12}, V_{22} )$,
								
								\vsitem[] \xblankpar \F{\m{D}^{\phantom{2D}}}{FW}$( X_{21}, U_{22}, V_{21} )$,~\F{\m{D}^{\phantom{2D}}}{FW}$( X_{22}, U_{22}, V_{22} )$
								
								\algobottomspace{}
							\end{enumerate}
							% \medskip\noindent{\func{\F{D}{FW} Ends}}
						}
					\end{minipage}
				\end{mycolorbox}
				\vspace{-0.2cm}
			\end{minipage} 
			\vspace{-0.1cm}
			\caption{{\small A recursive divide-and-conquer Floyd-Warshall algorithm.}}
			\label{fig:cofw}
		\end{center}
		% \end{minipage}
		\vspace{-0.4cm}
	}
\end{figure}


\begin{theorem}[\highlighttitle{Hybrid FW}]
	\label{thm:hybridfw}
	The hybrid FW algorithm, assuming a tall cache, has a complexity of $T_1(n) = \Th{n^3}$, $Q_1^{RELEASE}(n) = \Oh{n^3/(B\sqrt{M})}$\\ $Q_1^{RETAIN}(n) = \Oh{n^3/(B\sqrt{M}) + 2^k n^2 / B + 4^k n}$, \\ $S(n) = \Oh{2^k n^2}$, and $T_{\infty}(n) = \Oh{ n \log^2 (n/2^k) + k 2^k \log n }$.

\end{theorem}
\begin{proof}
The recurrences are:
	\vspace{-0.3cm}
	\begin{center}
	\scalebox{0.8}
	{
		\begin{minipage}{0.49\textwidth}
	\begin{align*}
	Q_{\m{A}}(m) &=  Q_{\m{B}}(m) = Q_{\m{C}}(m) = Q_{\m{D}}(m) \\
	&= \Oh{\frac{(n/2^k)^3}{B\sqrt{M}} + \frac{(n/2^k)^2}{B} + (n/2^k)} & \textrm{if $m = \frac{n}{2^k}$,} \\	
	Q_{\m{A}}(m) &=  
	2\left(
	\begin{array}{c}
	Q_{\m{A}}\left({m \over 2}\right) + Q_{\m{B}}\left({m \over 2}\right) \\
	+ Q_{\m{C}}\left({m \over 2}\right) + Q_{\m{D}}\left({m \over 2}\right) 
	\end{array}
	\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
	Q_{\m{B}}(m) &= 4 \left( Q_{\m{B}}\left({m \over 2}\right) + Q_{\m{D}}\left({m \over 2}\right) \right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
	Q_{\m{C}}(m) &= 4 \left( Q_{\m{C}}\left({m \over 2}\right) + Q_{\m{D}}\left({m \over 2}\right) \right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
	Q_{\m{D}}(m) &= 8Q_{\m{D}}\left({m \over 2}\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}
	\end{align*}
\end{minipage}
}
\end{center}
\vspace{-0.3cm}
\begin{center}
	\scalebox{0.8}
	{
		\begin{minipage}{0.49\textwidth}
			\begin{align*}
			T_{\m{A}}(m) &= \Th{(n/2^k) \log^2 (n/2^k)} & \textrm{if $m = n/2^k$,} \\
			T_{\m{B}}(m) &= T_{\m{C}}(m) = \Th{(n/2^k) \log (n/2^k)} & \textrm{if $m = n/2^k$,} \\
			T_{\m{D}}(m) &= \Th{n/2^k} & \textrm{if $m = n/2^k$,} \\
			T_{\m{A}}(m) &= 2\left(
			\begin{array}{c}
			T_{\m{A}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \\
			+ \max{\{ T_{\m{B}}\left({m \over 2}\right), T_{\m{C}}\left({m \over 2}\right) \}}
			\end{array}
			\right) + \Th{\log m} & \textrm{if $m > n/2^k$.}\\
			T_{\m{B}}(m) &= 2\left( T_{\m{B}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \right) + \Th{\log m} & \textrm{if $m > n/2^k$.}\\
			T_{\m{C}}(m) &= 2\left( T_{\m{C}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \right) + \Th{\log m} & \textrm{if $m > n/2^k$.}\\
			T_{\m{D}}(m) &= T_{\m{D}}\left({m \over 2}\right) + \Th{\log m} & \textrm{if $m > n/2^k$.}
			\end{align*}	
		\end{minipage}
	}
\end{center}
\vspace{-0.3cm}
\begin{center}
	\scalebox{0.8}
	{
\begin{minipage}{0.49\textwidth}
	\begin{equation*}
	S(n) = \sum_{i = 0}^{k - 1} 8^i \left( \frac{n}{2^i} \times \frac{n}{2^i} \right) = \Th{2^k n^2}
	\end{equation*}
	\end{minipage}
}
	\end{center}
	Solving the recurrences, we have the theorem.
\end{proof}

\subsubsection{Protein accordion folding}
The protein accordion folding (PF) is defined as follows. A protein is folded into a $2$-D square
lattice in such a way that the number of pairs of hydrophobic amino acids that are (vertically or horizontally) next to each other in the grid without being next to each other in the protein sequence is maximized. We assume that the fold is
always an {\em accordion fold} where the sequence first goes straight down, then straight
up, then again straight down, and so on. Further details related to the problem and a recursive divide-and-conquer algorithm for PF is given in \cite{TithiGaTaAgCh2015}. The algorithm has four functions $\m{A}, \m{B}, \m{C}$, and $\m{D}$. Due to space constraints, we do not give the algorithm here. The $\m{D}$ function in the algorithm is matrix-multiplication-like and dominates the total work complexity. Hence, by simply modifying the $\m{D}$ function to use extra space, we end up with not-in-place PF algorithm. 

\begin{figure}[ht!]
	\begin{center}
		\vspace{-0.1cm}
		\begin{minipage}{0.48\textwidth}
			\begin{mycolorbox}{\F{\m{A}}{PF}$(X)$}
				\begin{minipage}{0.98\textwidth}
					{\tiny
						\algotopspace{}
						\noindent
						\begin{enumerate}
							\setlength{\itemindent}{-2em}
							
							\vsitem \xif $X$ is a small matrix \xthen \L{\m{A}}{PF}$(X)$
							
							\vsitem \xelse
							
							\vsitem \T \F{\m{A}}{PF}$(X_{22})$
							\vsitem \T \F{\m{B}}{PF}$(X_{12},X_{22})$
							\vsitem \T \F{\m{C}}{PF}$(X_{11},X_{12})$
							\vsitem \T \F{\m{A}}{PF}$(X_{11})$
							
							\algobottomspace{}
						\end{enumerate}
						%\medskip\noindent{\func{\F{A}{FW} Ends}}
					}
				\end{minipage}
			\end{mycolorbox}
			\vspace{0.1cm}
			\begin{mycolorbox}{\F{\m{B}}{PF}$(X,V)$}
				\begin{minipage}{0.98\textwidth}
					{\tiny
						\algotopspace{}
						\noindent
						\begin{enumerate}
							\setlength{\itemindent}{-2em}
							
							\vsitem \xif $X$ is a small matrix \xthen \L{\m{B}}{PF}$(X,V)$
							
							\vsitem \xelse
							
							\vsitem \T \xpar \F{\m{B}}{PF}$(X_{11},V_{11})$, \F{\m{B}}{PF}$(X_{12},V_{22})$, \vsitem[] \xblankpar \F{\m{B}}{PF}$(X_{21},V_{11})$, \F{\m{B}}{PF}$(X_{22},V_{22})$
							
							\vsitem \T \xpar \F{\m{D}}{PF}$(X_{11},V_{12})$, \F{\m{D}}{PF}$(X_{21},V_{12})$
							
							\algobottomspace{}
						\end{enumerate}
						%\medskip\noindent{\func{\F{B}{FW} Ends}}
					}
				\end{minipage}
			\end{mycolorbox}
			\vspace{0.1cm}
			\begin{mycolorbox}{\F{\m{C}}{PF}$(X,U)$}
				\begin{minipage}{0.98\textwidth}
					{\tiny
						\algotopspace{}
						\noindent
						\begin{enumerate}
							\setlength{\itemindent}{-2em}
							
							\vsitem \xif $X$ is a small matrix \xthen \L{\m{C}}{PF}$(X,U)$
							
							\vsitem \xelse
							
							\vsitem \T \xpar \F{\m{C}}{PF}$(X_{11},U_{11})$, \F{\m{D}}{PF}$(X_{12},U_{21})$, \F{\m{C}}{PF}$(X_{22},U_{21})$
							
							\vsitem \T \xpar \F{\m{C}}{PF}$(X_{11},U_{12})$, \F{\m{D}}{PF}$(X_{12},U_{22})$, \F{\m{C}}{PF}$(X_{22},U_{22})$
							
							\algobottomspace{}
						\end{enumerate}
						% \medskip\noindent{\func{\F{D}{FW} Ends}}
					}
				\end{minipage}
			\end{mycolorbox}
			\vspace{0.1cm}
			\begin{mycolorbox}{\F{\m{D}}{PF}$(X,V)$}
				\begin{minipage}{0.98\textwidth}
					{\tiny
						\algotopspace{}
						\noindent
						\begin{enumerate}
							\setlength{\itemindent}{-2em}
							
							\vsitem \xif $X$ is a small matrix \xthen \L{\m{D}}{PF}$(X,V)$
							
							\vsitem \xelse
							
							\vsitem \T \xpar \F{\m{D}}{PF}$(X_{11},V_{11})$, \F{\m{D}}{PF}$(X_{12},V_{21})$,
							\vsitem[] \xblankpar \F{\m{D}}{PF}$(X_{21},V_{11})$, \F{\m{D}}{PF}$(X_{22},V_{21})$
							
							\vsitem \T \xpar \F{\m{D}}{PF}$(X_{11},V_{12})$, \F{\m{D}}{PF}$(X_{12},V_{22})$,
							\vsitem[] \xblankpar \F{\m{D}}{PF}$(X_{21},V_{12})$, \F{\m{D}}{PF}$(X_{22},V_{22})$
							
							\algobottomspace{}
						\end{enumerate}
						%\medskip\noindent{\func{\F{C}{FW} Ends}}
					}
				\end{minipage}
			\end{mycolorbox}
		\end{minipage}
		\vspace{-0.3cm}
		\caption{A recursive divide-and-conquer algorithm for the protein accordion folding problem.}
		\label{fig:copf}
	\end{center}
	% \end{minipage}
	\vspace{-0.4cm}
	%\end{wrapfigure}
\end{figure}


\begin{theorem}[\highlighttitle{Hybrid PF}]
	\label{thm:hybridpf}
	The hybrid PF algorithm, assuming a tall cache, has a complexity of $T_1(n) = \Th{n^3}$, $Q_1^{RELEASE}(n) = \Oh{n^3/(B\sqrt{M})}$, \\ $Q_1^{RETAIN}(n) = \Oh{n^3/(B\sqrt{M}) + 2^k n^2 / B + 4^k n}$, \\$S(n) = \Oh{2^k n^2}$,\\$\text{and }T_{\infty}(n) = \Oh{ 
		n \left( \log (n/2^k) + k/2^k \right) + k 2^k (\log n - k)}$
	
\end{theorem}
\begin{proof}
	The recurrences are:
	\vspace{-0.3cm}
	\begin{center}
		\scalebox{0.8}
		{
			\begin{minipage}{0.49\textwidth}
				\begin{align*}
				Q_{\m{A}}(m) &=  Q_{\m{B}}(m) = Q_{\m{C}}(m) = Q_{\m{D}}(m) \\
				&= \Oh{\frac{(n/2^k)^3}{B\sqrt{M}} + \frac{(n/2^k)^2}{B} + (n/2^k)} & \textrm{if $m = \frac{n}{2^k}$,} \\	
				Q_{\m{A}}(m) &=  2 Q_{\m{A}}\left({m \over 2}\right) +  Q_{\m{B}}\left({m \over 2}\right) +  Q_{\m{C}}\left({m \over 2}\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
				Q_{\m{B}}(m) &= 4 Q_{\m{B}}\left({m \over 2}\right) + 2 Q_{\m{D}}\left({m \over 2}\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
				Q_{\m{C}}(m) &= 4 Q_{\m{C}}\left({m \over 2}\right) + 2 Q_{\m{D}}\left({m \over 2}\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}\\
				Q_{\m{D}}(m) &= 8Q_{\m{D}}\left({m \over 2}\right) + \Th{\frac{m^2}{B} + m} & \textrm{if $m > \frac{n}{2^k}$.}
				\end{align*}
			\end{minipage}
		}
	\end{center}
	\vspace{-0.3cm}
	\begin{center}
		\scalebox{0.8}
		{
			\begin{minipage}{0.49\textwidth}
				\begin{align*}
				T_{\m{A}}(m) &= \Th{(n/2^k) \log^2 (n/2^k)} & \textrm{if $m = n/2^k$,} \\
				T_{\m{B}}(m) &= T_{\m{C}}(m) = \Th{(n/2^k) \log (n/2^k)} & \textrm{if $m = n/2^k$,} \\
				T_{\m{D}}(m) &= \Th{n/2^k} & \textrm{if $m = n/2^k$,} \\
				T_{\m{A}}(m) &= 2\left(
				\begin{array}{c}
				T_{\m{A}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \\
				+ \max{\{ T_{\m{B}}\left({m \over 2}\right), T_{\m{C}}\left({m \over 2}\right) \}}
				\end{array}
				\right) + \Th{1} & \textrm{if $m > n/2^k$.}\\
				T_{\m{B}}(m) &= 2\left( T_{\m{B}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \right) + \Th{\log m} & \textrm{if $m > n/2^k$.}\\
				T_{\m{C}}(m) &= 2\left( T_{\m{C}}\left({m \over 2}\right) + T_{\m{D}}\left({m \over 2}\right) \right) + \Th{\log m} & \textrm{if $m > n/2^k$.}\\
				T_{\m{D}}(m) &= T_{\m{D}}\left({m \over 2}\right) + \Th{\log m} & \textrm{if $m > n/2^k$.}
				\end{align*}	
			\end{minipage}
		}
	\end{center}
	\vspace{-0.3cm}
	\begin{center}
		\scalebox{0.8}
		{
			\begin{minipage}{0.49\textwidth}
				\begin{equation*}
				S(n) = \sum_{i = 0}^{k - 1} 8^i \left( \frac{n}{2^i} \times \frac{n}{2^i} \right) = \Th{2^k n^2}
				\end{equation*}
			\end{minipage}
		}
	\end{center}
	Solving the recurrences, we have the theorem.
\end{proof}





==> dump.tex <==
\newpage{}
-----------------------------------\\


\hide{

\begin{figure*}
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{Compute-Output-Arrays}(y, \text{stage\_id, root\_id})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem height $\gets$ \#levels in the stage; \#leaves $\gets 2^{\text{height}}$ 

\vsitem \xparallelfor node $\gets 0$ \xto \#leaves $-1$ \xdo
\vsitem \T leaf\_id $\gets$ (root\_id $- 1$) $\times$ \#leaves $+ $ node 
\vsitem \T \xif last stage \xthen $y$[stage\_id][leaf\_id][0] $\gets$ $a$[stage\_id][leaf\_id][0]
\vsitem \T \xelse \textsc{Compute-Output-Arrays}$(y, \text{stage\_id + 1, leaf\_id})$

\vsitem \xparallelfor $i \gets 0$ \xto $n-1$ \xdo \label{line:spawnoutputcells-fft}
\vsitem \T  \textsc{Compute-Output-Cell}($y$, stage\_id, root\_id, $i, n$, height)

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Output-Cell}(y, \text{stage\_id, node\_id, $i, n$, height})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif height $= 0$ \xthen \xreturn $a$[stage\_id + 1][node\_id][$i$]

\vsitem \xparallelfor $k \gets 0$ \xto $1$ \xdo
\vsitem \T child\_id $\gets$ (node\_id $- 1$) $\times 2 + k$
\vsitem \T $t[k] \gets 0$; coeff $\gets$ \textcolor{red}{?}
\vsitem \T new\_$i$ $\gets$  \textcolor{red}{?}
\vsitem \T $t[k] \gets$ coeff $\times$ \textsc{Compute-Output-Cell}($y$, stage\_id, child\_id, new\_$i$, $n/2$, height $- 1$)
\vsitem \xreturn $t[0] + t[1]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\caption{The 2-way \textsc{FFT} algorithm.}
\label{fig:fft-pseudocode-2way}
\vspace{-0.2cm}
\end{figure*}





%--------------------

$[$Work.$]$ We compute the required DFT in $h$ \bands $S_0, S_1, \ldots, S_{h - 1}$, where $h = 1/ \psi$. Suppose $W_i$ defines the work done at \band $S_i$. We first come up with a generic formula for $W_i$. We use a direct proof to show that $W_i = \Oh{n^{1 + \psi}}$, which implies that the total work is $\sum_{i = 0}^{h - 1} W_i = \Oh{(1/\psi) n^{1 + \psi}}$.

We compute $W_i$ for $i \in [0, h - 1]$. Each DFT at the root level of stage $S_i$ is constructed from the DFT's at the leaf level of the stage. All cells in all DFT's at the root level of stage $S_i$ are computed in parallel. \#Nodes at the root level of \band $S_i$ is $2^{i\psi \log n} = n^{i\psi}$. Each such DFT has $n/2^{i \psi \log n} = n^{1 - i\psi}$ cells. Each cell at a recursion level $\ell$ depends on exactly $2$ DFT cells in recursion level $\ell +1$. Hence, each cell in the DFT at the root level of stage $S_i$ depends on $\mathcal{O}(2^{\psi \log n}) = \Oh{n^{\psi}}$ cells in the DFT at the leaf level of the stage. Hence, $W_i = \Oh{n^{i \psi} n^{1 - i\psi} n^{\psi}} = \Oh{n^{1 + \psi}}$ for all $i \in [0, h - 1]$. Combining the work of all \bands, we get $T_1(n) = \sum_{i = 0}^{h - 1} W_i = \Oh{(1/\psi) n^{1 + \psi}}$.

\okay{}

\vspace{0.1cm}
\noindent
[Span.] Let $T_{\infty}(m, i)$ denote the span to compute the $m$-sized DFT array at the root level of stage $i$. We give a recursive formula to compute $T_{\infty}(m, i)$. Then, the total span for the algorithm is $T_{\infty}(n, 0)$.

\#Nodes at the leaf level of stage $S_i$ is $n^{(i + 1)\psi \log n}$. Launching these nodes in parallel incurs a span of $\Oh{i \psi \log^2 n}$. An array at the leaf level will be of size $m/2^{\psi \log n} = m / n^{\psi}$. Spawning single-point evaluation function \textsc{FFT-sp} for all cells (i.e., global synchronization) incurs a span of $\Oh{i \psi \log^2 n + \log (m/n^{\psi})}$. Executing the \textsc{Compute-Output-Cell} algorithm incurs $\Oh{\log \psi}$ span. Adding all these spans give us $\Oh{i \log \psi + \log m} = \Oh{\log (m\psi^i)}$.

The span of stage $S_i$ recursively depends upon the span of stage $S_{i + 1}$ as the output arrays at the leaf level of stage $S_{i + 1}$ are constructed from the leaf level arrays of stage $S_{i}$. Hence, $T_{\infty}(m,i)$ can be recursively defined using the previous analysis as:
$T_{\infty}(m,i) = \Oh{\log \psi}$ if $i = h$ and $T_{\infty}(m,i) = \Oh{\log (m\psi^i)} + T_{\infty}(m/\psi,i+1)$ if $i < h$.

By unrolling the recursion and simplifying, we compute the total span as $T_{\infty}(n,0) = \Oh{\log^2 n / \log \psi}$.\\
 
\vspace{-0.2cm}
\noindent
[Space.] The space requirement at each stage is $\Oh{n}$ and there are $\log n / \log \psi$ stages. Hence, the total space is $\Oh{n \log n / \log \psi}$.



%We consider the \textit{work-span model} \cite{CormenLeRiSt2009}, sometimes called the fork-join model, to analyze the performance of shared-memory parallel programs. In this model, $T_1(n)$ and $T_{\infty}(n)$ represent the running times on an algorithm with input parameter $n$ on 1- and $\infty$-processor machines, respectively. We use the \textit{ideal cache model} \cite{frigo2012cache} to analyze the cache performance. As per the model, $Q_1(n)$ represents the total number of data block transfers between adjacent levels of memory.

The recurrences for  are:\\
\scalebox{0.8}
{
\centering
\begin{minipage}{0.49\textwidth}
\begin{align*}
& T_1^{TF}(n) = T_{\infty}^{TF}(n) = S_{\infty}^{TF}(n) = \Th{1} \qquad \text{if } n = 1,\\
& T_1^{TF}(n) = 2^{(s + s')} T_1^{TF}(n / 2) + \Th{1} \qquad \text{if } n > 1.\\
& T_{\infty}^{TF}(n) = T_{\infty}^{TF}(n / 2) + \Th{s + s'} \qquad \text{if } n > 1.\\
& S_{\infty}^{TF}(n) = 2^{(s + s')} S_{\infty}^{TF}(n / 2) + \Th{1} \qquad \text{if } n > 1.\\
&Q_1^{TF}(n) = \begin{cases} \Th{n^{(s + s')}/B + n^{(s + s' - 1)}} &\mbox{if } n^{s + s'} \le \alpha M,\\ 
2^{s + s'} Q_1^{TF}(n / 2) + \Th{1}  & \mbox{if } n^{s + s'} > \alpha M. \end{cases}
\end{align*}    
\end{minipage}
}\\

\paragraph{Invariant: } Suppose that we are multiplying two matrices $a\cross b$ and $b\cross c$ using $r$ planes each of size $a\cross c$. Then, when the value of $a$ reaches the value of $b$, then the final value of $a$ remains the same with the final value of $b$ when $r=1$.



\begin{mycolorbox}{$\textsc{TF}(M,T,s, s')$ \xcomment Tensor Flattening}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem \xparallelfor $i_1 \leftarrow 1$ \xto $n$ \xdo
\vsitem $\cdots$
\vsitem \xparallelfor $i_s \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \xparallelfor $j_1 \leftarrow 1$ \xto $n$ \xdo
\vsitem \T $\cdots$
\vsitem \T \xparallelfor $j_{s'} \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \T $I \gets \textsc{Linearize}(i_1, \ldots, i_s)$ \xcomment $I \in [1, n^s]$
\vsitem \T \T $J \gets \textsc{Linearize}(j_1, \ldots, j_{s'})$  \xcomment $J \in [1, n^{s'}]$
%\vsitem \T \T $[I, J] \gets [\sum_{k=1}^s (i_k - 1) \cdot n^{s-k}, \sum_{k=1}^{s'} (j_k - 1) \cdot n^{s'-k}]$
\vsitem \T \T $M[I,J] \gets T[i_1, \ldots, i_s, j_1, \ldots, j_{s'}]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}



\vspace{-0.2cm}
\begin{mycolorbox}{$\textsc{TC-MM-Naive}(X,U,V)$ \xcomment In-place}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\vspace{0.1cm}
\algorequire $u, v, x \ge 1$
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem \xparallelfor $i_1 \leftarrow 1$ \xto $n$ \xdo
\vsitem $\cdots$
\vsitem \xparallelfor $i_{u - 1} \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \xparallelfor $j_1 \leftarrow 1$ \xto $n$ \xdo
\vsitem \T $\cdots$
\vsitem \T \xparallelfor $j_{v - 1} \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \T \xfor $k_1 \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \T $\cdots$
\vsitem \T \T \xfor $k_{x - 1} \leftarrow 1$ \xto $n$ \xdo
\vsitem \T \T \T $\textsc{MM}(X_{i_1..i_{u - 1},i_u[1..n], j_1..j_{v - 1}, j_v[1..n]}$,
\vsitem[] \T \T \T \T $U_{\{i_1..i_{u - 1},i_u[1..n],k_1..k_{x - 1}, k_x[1..n]\}}$,
\vsitem[] \T \T \T \T  $V_{\{j_1..j_{v - 1}, j_v[1..n],k_1..k_{x - 1}, k_x[1..n]\}})$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
}


{\large \textbf{\textcolor{red}{DO NOT READ FROM HERE}}}\\
\cite{FrigoLePrRa1999, Tang2017} 

\begin{theorem}[\highlighttitle{Hybrid TC}]
	\label{thm:hybridtc}
	The hybrid TC algorithm $\textsc{TC-HS}$ has a complexity of $T_1(n) = \Th{n^{w}}$, $Q_1^{RELEASE}(n) = \Th{n^{r+z}/BM^{((r+z)/s) -1}}$, \\ $Q_1^{RETAIN}(n) = \Th{n^{r+z}/BM^{((r+z)/s) -1} + (2^{rk}n^z)/B}$ \\ where $s = max(x,y,z)$; if $(r + z\log n) = \omega(\log n)$, then $T_{\infty}(n)=\Th{r + z\log n}$  otherwise $\Th{\log^{2}n}$, and $S(n) = \Th{2^{rk}n^z}$.
\end{theorem}
\begin{proof}
	In the hybrid TP algorithm \F{\m{A}}{TP\textrm{-}H}, when the size of each dimension of input tensor drops to $n / 2^k$ or below then we execute \F{\m{A}}{TP}. Hence, in the following recurrences, when the problem size reaches the base case (i.e., when $m = n / 2^k$), the complexities are same as the complexities from Lemma \ref{lem:inplacetc} but $n$ is replaced by $n / 2^k$. Also, the recursion cases are from Lemma \ref{lem:inplacetc}. Thus, we have:
	\begin{center}
		\scalebox{0.8}
		{
			\begin{minipage}{0.49\textwidth}
			\begin{align*}
			T_1(m) &= \begin{cases} \Th{(n/2^k)^z+r} &\mbox{if } m = n/2^k, \\ 
			2^{z+r}T_{1}(\frac{m}{2}) + \Th(2^{r}n^{z})  & \mbox{if } m > n/2^k. \end{cases}\\
			Q_1(m) &= \begin{cases} \Th{(n/2^k)^{x}/B + (n/2^k)^{y}/B + (n/2^k)^{z}/B + 1} &\mbox{if } m = n/2^k, \\ 
			2^{z+r}Q_{1}(m/2) + \Th{2^{r}m^{z}/B + 1}  & \mbox{if } m > n/2^k. \end{cases}\\
			T_{\infty}(m) &= \begin{cases} \Th{m/2^k} &\mbox{if } m = n/2^k, \\ 
			2^{r}T_{\infty}(\frac{m}{2}) + \Th{r + z\log m} & \mbox{if } m > n/2^k. \end{cases}\\
			S(n) &= \begin{cases} \Th{(n/2^k)^z} &\mbox{if } m = n/2^k, \\ 
			2^{z+r}(n/2) + \Th{2^{r}m^z}  & \mbox{if } m > n/2^k. \end{cases}
			\end{align*}
			\end{minipage}
		}
	\end{center}	
	
\end{proof}

We now design a full not-in-place algorithm that uses $\Th{n^w}$ total space and processors.

\begin{lemma}[\highlighttitle{Full not-in-place TC}]
	\label{lem:notinplacetp}
	The full not-in-place TC algorithm has a complexity of $T_1(n) = \Th{n^{w}}$, $T_{\infty}(n)=\Th{w \log n}$, $S_{\infty}(n) = \Th{n^{w}}$, and $Q_1(n) = \Th{n^{w}/B}$.
\end{lemma}
\begin{proof}
The recurrences for the complexities are as follows:
\begin{center}
\scalebox{0.8}
{
\begin{minipage}{0.49\textwidth}
\begin{align*}
& T_1(n) = T_{\infty}(n) = S_{\infty}(n) = \Th{1} \qquad \text{if } n = 1,\\
& T_1(n) = 2^w T_1(n / 2) + \Th{1} \qquad \text{if } n > 1.\\
& T_{\infty}(n) = T_{\infty}(n / 2) + \Th{w} \qquad \text{if } n > 1.\\
& S_{\infty}(n) = 2^{w} S_{\infty}(n / 2) + \Th{1} \qquad \text{if } n > 1.\\
&Q_1(n) = \begin{cases} \Th{tspace/B + tspace/n} &\mbox{if } tspace \le \alpha M,\\ 
2^{w} Q_1(n / 2) + \Th{1}  & \mbox{if } tspace > \alpha M. \end{cases}
\end{align*}    
\end{minipage}
}
\end{center}
\end{proof}




 
\begin{lemma}[\highlighttitle{TC-MM}]
	\label{lem:tc-mm}
	The TC-MM algorithm has a complexity of $T_1(n) = \Th{n^{w}}$, $T_{\infty}(n)=\Th{n^{x}}$, $S_{\infty}(n) = \Th{n^{s}}$, and $Q_1(n) = \Th{n^{w-3}\left(n^3/(B\sqrt{M}) + n^3 + n^2/B + n + 1\right)}$.
\end{lemma}
\begin{proof}
TC-MM is an iterative procedure that calls MM $n^{w-3}$ times, in serial blocks $n^{x}$ long. Therefore $T_{\infty}(n)$ and $Q_1(n)$ reflect MM's complexities respectively multiplied by $n^{x}$ and $n^{w-3}$.

MM takes matrices with either row- or column-major ordering, so we reorder the indices of $U$ and $V$ prior to the core of TC-MM, and we reorder $X$ afterward. These tensor transpositions incur a complexity of $T_1(n) = \Th{n^{s}}$, $T_{\infty}(n)=\Th{1}$, $S_{\infty}(n) = \Th{n^{s}}$, and $Q_1(n) = \Th{n^{s}/B}$.
\end{proof}

\begin{lemma}[\highlighttitle{TC-MM-2}]
	\label{lem:tc-mm-2}
	The TC-MM-2 algorithm has a complexity of $T_1(n) = \Th{n^w}$, $T_{\infty}(n)=\Th{n^s}$, $S_{\infty}(n) = \Th{n^s}$, and $Q_1(n) = \Th{n^w/(B \sqrt{M}) + n^w/M + n^s / B + n^u + n^v + n^x + 1}$.
\end{lemma}
\begin{proof}
TC-MM-2 is a single MM call wrapped in code to flatten $U$ and $V$, and restructure $X$. This is equivalent to rearranging their indices, so the complexity of everything except the call to MM is given by $T_1(n) = \Th{n^{s}}$, $T_{\infty}(n)=\Th{1}$, $S_{\infty}(n) = \Th{n^{s}}$, and $Q_1(n) = \Th{n^{s}/B}$. The complexity of the MM call itself on matrices of size $n^u \times n^v$, $n^u \times n^x$, and $n^x \times n^v$, is $T_1(n) = \Th{n^w}$, $T_{\infty}(n)=\Th{n^s}$, $S_{\infty}(n) = \Th{n^s}$, and $Q_1(n) = \Th{n^w/(B \sqrt{M}) + n^w/M + n^s / B + n^u + n^v + n^x + 1}$. (see \cite{prokop1999cache}).
\end{proof}

\subsection{Hybrid algorithm for matrix multiplication}
The \F{\m{A}}{MM} algorithm has optimal cache complexity from Lemma \ref{lem:inplacemm} and the \F{\m{A}}{MM\textrm{-}N} algorithm has very high parallelism from Lemma \ref{lem:notinplacemm}. Is it possible to develop a hybrid algorithm that has optimal serial cache complexity and highest parallelism? We take a step in this direction to develop a hybrid algorithm combining both \F{\m{A}}{MM} and \F{\m{A}}{MM\textrm{-}N} that has optimal serial cache complexity and has asymptotically more parallelism than that of \F{\m{A}}{MM}.
We propose a hybrid algorithm that executes \F{\m{A}}{MM\textrm{-}N} until the size of the input submatrix drops to $n / 2^k$ or below and then execute \F{\m{A}}{MM}. \\

The hybrid algorithm is interesting because it offers a tradeoff between cache complexity and parallelism. From hereon, we term this hybrid algorithm \F{\m{A}}{MM\textrm{-}H}, where $H$ refers to hybrid. The increase in parallelism comes with increase in the extra space used. We call this tradeoff the \highlight{space-parallelism tradeoff}.

\hide{
\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=0.2\textwidth]{hybrid-MM.pdf}
		\caption{Hybrid matrix multiplication algorithm.}
		\label{fig:hybridMMtheorem}
	\end{center}
\end{figure}
}

The hybrid MM algorithm \F{\m{A}}{MM\textrm{-}H} is shown in Figures \ref{fig:hybridMMtheorem} and \ref{fig:matrixmultiplication}. The algorithm starts with $m$ planes where each plane is an extra space of size $n\times n$. \F{\m{A}}{MM\textrm{-}H} calls itself recursively till $k$-th level of recursion and at each recursive call it specify the planes where temporary output will be written. This is denoted by specifying the starting plane number $s$ and number of planes $m$ allocated for a particular recursive call. The way the algorithm works is that we execute the not-in-place algorithm (i.e., \F{\m{A}}{MM\textrm{-}N}) until the problem size or the task size reduces to a threshold value, say $(n/2^k) \times (n/2^k)$ for some $k$, and then we execute the in-place algorithm (i.e., \F{\m{A}}{MM}). %The converse of the observation above, i.e., initially executing \F{\m{A}}{MM} and later \F{\m{A}}{MM\textrm{-}N} is not a good idea because even if we execute \F{\m{A}}{MM\textrm{-}N} at the end for only one level, we will have $S_{\infty}(n)$ will be $\Th{n^3}$ and hence $Q_1(n)$ will be $\Th{n^3 / B}$.

In \F{\m{A}}{MM\textrm{-}H}, the more number of levels we execute \F{\m{A}}{MM\textrm{-}N} initially, the more space we consume, the more parallelism we have, and more number of cache misses are incurred. Therefore, we need to carefully choose the level $k$ in which we need to switch from one algorithm to another. The complexity of the \F{\m{A}}{MM\textrm{-}H} algorithm is given in Theorem \ref{thm:hybridmm}.

%We implement this idea using statically allocated $n \times n$ sized grids or planes.

\begin{theorem}[\highlighttitle{Hybrid MM}]
	\label{thm:hybridmm}
	The hybrid MM algorithm\\ \F{\m{A}}{MM\textrm{-}H}, assuming a tall cache, has a complexity of\\ $T_1(n) = \Th{n^3}$, $Q_1^{RELEASE}(n) = \Oh{n^3/(B\sqrt{M}) + n^2 / B + n}$,\\ $Q_1^{RETAIN}(n) = \Oh{n^3/(B\sqrt{M}) + (2^k n^2)/B + n^2 / B + n}$, \\ $S(n) = \Oh{2^k n^2}$, and \\$T_{\infty}(n)=\Oh{k(2\log n - k)+n/2^k}$.
\end{theorem}
\begin{proof}
	In the hybrid MM algorithm \F{\m{A}}{MM\textrm{-}H}, when the size of each input matrix drops to $n / 2^k$ or below then we execute \F{\m{A}}{MM}. Hence, in the following recurrences, when the problem size reaches the base case (i.e., when $m = n / 2^k$), the complexities are same as the complexities from Lemma \ref{lem:inplacemm} but $n$ is replaced by $n / 2^k$. Also, the recursion cases are from Lemma \ref{lem:notinplacemm}. Thus, we have:
	\begin{center}
		\scalebox{0.8}
		{
			\begin{minipage}{0.49\textwidth}
	\begin{align*}
	T_1(m) &= \begin{cases} \Th{(n/2^k)^3} &\mbox{if } m = n/2^k, \\ 
	8 T_1(\frac{m}{2}) + \Th{1}  & \mbox{if } m > n/2^k. \end{cases}\\
	Q_1(m) &= \begin{cases} \Th{n^3 / (8^k B\sqrt{M}) + n^2/(4^k B) + n/2^k} &\mbox{if } m = n/2^k, \\ 
	8 Q_1(\frac{m}{2}) + \Th{\frac{m^2}{B} + m}  & \mbox{if } m > n/2^k. \end{cases}\\
	T_{\infty}(m) &= \begin{cases} \Th{n/2^k} &\mbox{if } m = n/2^k, \\ 
	T_{\infty}(\frac{m}{2}) + \Oh{\log m}  & \mbox{if } m > n/2^k. \end{cases}\\
	S(m) &= \begin{cases} \Oh{(n/2^k)^2} &\mbox{if } m = n/2^k, \\ 
	8 S(\frac{m}{2}) + \Th{m^2}  & \mbox{if } m > n/2^k. \end{cases}
	\end{align*}
	\end{minipage}
}
	\end{center}
\end{proof}



Theorem \ref{thm:hybridmm} may or may not be cache-efficient depending on the value of $k$. If we switch from not-in-place to in-place at large value of $k$, there will be more parallelism, but at the same time cache complexity will also increase. Lemma \ref{lem:efficienthybridmm} gives trade-off between cache complexity and parallelism.  


\begin{theorem}[\highlighttitle{Cache-optimal hybrid MM}]
	\label{lem:efficienthybridmm}
	The maximum ideal speedup \F{\m{A}}{MM\textrm{-}H} can attain with extra space $S$ and remaining cache optimal is \\ $\Oh{(n^3+S\sqrt{M})/\big(M^{3/2}\big(\log (S/n^2)\cdot \log (n^4/S) + n^3/S\big)\big)}$. 
\end{theorem}


\begin{proof}
In case of hybrid MM algorithm with extra space $S$, we need to switch from not-in-place to in-place version at level $k$ such that total extra space used by the algorithm matches $S$ i.e. $2^kn^2 = S$. Hence, $k = \log_{2}s/n^2$.  
\begin{equation}
\begin{aligned}
T_{\infty}(n) &= \Th{k(2\log n - k)+ n/2^k} \\
&= \Th{\log \frac{S}{n^2}. \log \frac{n^4}{S} + n^3/S}
\end{aligned}
\end{equation}

If we release the extra space at the end of algorithm, the serial cache complexity $Q_{1}$ will be as follows:
 \begin{equation}
 Q_{1}(n) = \Th{\frac{n^3}{B\sqrt{M}} + S/B}
  \end{equation}
  The parallel cache complexity $Q_{p}$ (p is the number of processor) will be as follows:
  \begin{equation}
  Q_{p}(n) = \Oh{Q_{1}+p\frac{M}{B}T_{\infty}}
  \end{equation}
  If we want $Q_{p} = \Oh{Q_{1}}$, then the following must be satisfied.
  
  \begin{equation}
  \begin{aligned}
  p &= \Oh{\frac{Q_{1}}{T_{\infty}}\frac{B}{M}} \\
  &= \Oh{\frac{\frac{n^3}{B\sqrt{M}}+\frac{S}{B}}{\log \frac{S}{n^2}. \log \frac{n^4}{S} + n^3/S}.\frac{B}{M}} \\
  &= \Oh{\frac{n^3+S\sqrt{M}}{M^{3/2}(\log \frac{S}{n^2}. \log \frac{n^4}{S} + n^3/S)}}
  \end{aligned}
  \end{equation}
  
 
 \end{proof}

\begin{lemma}
	\label{lem:tradeofftensor}
	Let $X$ be a order $x$ tensor, $Y$ be a order $y$ tensor. If their tensor product $Z = X\otimes Y$ be a order $x+y$ tensor i.e. there is no scope of contraction of dimension, then there is  no space-parallelism trade-off.
\end{lemma}

\begin{proof}
	In that case, the number of elementary operations is equal to the number of different spaces in $Z$ tensor. Hence there is no temporal locality resulting no trade-off between space and parallelism.  
\end{proof}

\hide{
Analogous to matrix multiplication 
Tensor product has many applications in physics\cite{feynman1963feynman}, chemistry\cite{valiev2010nwchem}, and engineering\cite{delmarcelle1994topology,anandkumar2014tensor}.
In tensor algebra, tensors can be represented as multi-dimensional matrices. A $k$-dimensional matrix can be represented as $A(a_{1},a_{2},\ldots,a_{k})$ where $a_{i}$ ($1\le i\le k$ ) represents the dimensions . For example a two dimensional matrix multiplication can be represented as $A(a,b)\times B(b,c) = C(a,c)$.  Here dimension $b$ gets contracted. Similarly, tensor $X$ of order $k$ is a $k$ dimensional matrix. Unlike two dimensional matrix multiplication, in tensor product, more than one dimension can be contracted or may be no dimension gets contracted.  For example, doing a tensor product between a order 4 tensor $A(a,b,c,d)$ and order 3 tensor $B(c,d,e)$, the resultant tensor will be $C(a,b,e)$. Here both $c$ and $d$ dimensions get contracted. On the contrary, if $A(a,b,c,d)\otimes B(e,f,g) = C(a,b,c,d,e,f,g)$, then there is no contraction of dimension. 
}


==> figures.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\textwidth]{stages.pdf}
\caption{Stages in the \textsc{Strassen-S} MM algorithm for computing the input matrices.}
\label{fig:strassen-stages}
\end{figure}

\begin{figure}[!ht]
\centering
\begin{minipage}{\textwidth}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=\textwidth]{precomputation.pdf}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=\textwidth]{reduction.pdf}
\end{minipage}
\end{minipage}
\caption{\small Left: Single-point computation of a cell in the input matrix $U$ at a leaf node in a stage. Right: Single-point computation of a cell in the output matrix $X$ at a root node in a stage. (If there is an arrow from cell $a$ to cell $b$, it means that cell $a$ depends on cell $b$.)}
\label{fig:strassen-singlepoint-computation}
\end{figure}

\begin{figure*}[!ht]
\centering
\begin{minipage}{\textwidth}
{\scriptsize
\centering
\begin{minipage}{0.6\textwidth}
% Uquad
\centering
\begin{colortabular}{c | c c}
 & $k = 0$ & $k = 1$\\
\rowcolor{tabletitlecolor} \rotatebox{90}{branch\_id} & $\langle$ \rotatebox{90}{shift\_i}, \rotatebox{90}{shift\_j}, \rotatebox{90}{coeff} $\rangle$ & $\langle$ \rotatebox{90}{shift\_i}, \rotatebox{90}{shift\_j}, \rotatebox{90}{coeff} $\rangle$ \\ \hline
$0$ & $\langle 0, 0, 1 \rangle$ & $\langle 1, 1, 1 \rangle$ \\
$1$ & $\langle 1,0,1 \rangle$ & $\langle 1,1,1 \rangle$ \\
$2$ & $\langle 0,0,1 \rangle$ & $\langle -,-,0 \rangle$ \\
$3$ & $\langle 1,1,1 \rangle$ & $\langle -,-,0 \rangle$ \\
$4$ & $\langle 0,0,1 \rangle$ & $\langle 0,1,1 \rangle$ \\
$5$ & $\langle 1,0,1 \rangle$ & $\langle 0,0,-1 \rangle$ \\
$6$ & $\langle 0,1,1 \rangle$ & $\langle 1,1,-1 \rangle$ \\
\end{colortabular}
%Vquad
\begin{colortabular}{c|cc}
 & $k = 0$ & $k = 1$\\
\rowcolor{tabletitlecolor} \rotatebox{90}{branch\_id} & $\langle$ \rotatebox{90}{shift\_i}, \rotatebox{90}{shift\_j}, \rotatebox{90}{coeff} $\rangle$ & $\langle$ \rotatebox{90}{shift\_i}, \rotatebox{90}{shift\_j}, \rotatebox{90}{coeff} $\rangle$ \\ \hline
$0$ & $\langle 0,0,1 \rangle$ & $\langle 1,1,1 \rangle$ \\
$1$ & $\langle 0,0,1 \rangle$ & $\langle -,-,0 \rangle$ \\
$2$ & $\langle 0,1,1 \rangle$ & $\langle 1,1,-1 \rangle$ \\
$3$ & $\langle 1,0,1 \rangle$ & $\langle 0,0,-1 \rangle$ \\
$4$ & $\langle 1,1,1 \rangle$ & $\langle -,-,0 \rangle$ \\
$5$ & $\langle 0,0,1 \rangle$ & $\langle 0,1,1 \rangle$ \\
$6$ & $\langle 1,0,1 \rangle$ & $\langle 1,1,1 \rangle$ \\
\end{colortabular}
\end{minipage}
\begin{minipage}{0.4\textwidth}
% Xbranch
\centering
\begin{colortabular}{c|ccccccc|}
& \multicolumn{7}{c|}{$k$} \\
\rowcolor{tabletitlecolor}  \rotatebox{90}{quad\_id} & 0 & 1 & 2 & 3 & 4 & 5 & 6 \\ \hline
$0$ & $1$ & $0$ & $0$ & $1$ & $-1$ & $0$ & $1$\\
$1$ & $0$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$\\
$2$ & $0$ & $1$ & $0$ & $1$ & $0$ & $0$ & $0$\\
$3$ & $1$ & $-1$ & $1$ & $0$ & $0$ & $1$ & $0$\\
\end{colortabular}
\end{minipage}
}
\end{minipage}
\vgap{}
\caption{Data structures required for the \textsc{Strassen-S} MM algorithm. Left: $Uquad$ and $Vquad$. Right: $Xbranch$.}
\label{fig:strassen-algorithm-ds}
\end{figure*}

\begin{figure*}[!ht]
\centering
\scalebox{0.94}{
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{Strassen-S}(X, U, V)$ \xcomment $X \gets U \times V$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem ($\overline{U}, \overline{V}, \overline{X}$, $U$quad, $V$quad, $X$branch) $\gets$ \textsc{Construct-Data-Structures}($U, V$)
\vsitem \textsc{Compute-Input-Matrices}($\overline{U}, 0, 0$, $U$quad);  \textsc{Compute-Input-Matrices}($\overline{V}, 0, 0$, $V$quad)
\vsitem \textsc{Compute-Output-Matrices}($\overline{X}, 0, 0$, $X$branch)
\vsitem $X \gets \overline{X}[0][0]$ 

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Input-Matrices}(Z, \text{stage\_id, root\_id, quad})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem height $\gets$ \#levels in the stage; \#leaves $\gets 7^{\text{height}}$ 
\vsitem \xparallelfor node $\gets 0$ \xto \#leaves $-1$ \xdo \label{line:leafnodeslaunching}
\vsitem \T leaf\_id $\gets$ (root\_id $- 1$) $\times$ \#leaves $+ $ node 
\vsitem \T \xparallelfor $i \gets 0$ \xto $n-1$ \xdo \label{line:spawninputrows}
\vsitem \T \T \xparallelfor $j \gets 0$ \xto $n-1$ \xdo \label{line:spawninputcols}
\vsitem \T \T \T $Z$[stage\_id][leaf\_id][$i, j$] $\gets$  \textsc{Compute-Input-Cell}($Z$, stage\_id, leaf\_id, $i, j, n$, height, quad)
\vsitem \T \xif not last stage \xthen \textsc{Compute-Input-Matrices}($Z$, stage\_id + 1, leaf\_id, quad)
		
\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Input-Cell}(Z, \text{stage\_id, node\_id, $i, j, n$, height, quad})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem \xif height $= 0$ \xthen \xreturn $Z$[stage\_id][node\_id][$i, j$]
\vsitem parent\_id $\gets$ (node\_id $/$ 7), branch\_id $\gets$ node\_id mod 7
\vsitem \xparallelfor $k \gets 0$ \xto $1$ \xdo
\vsitem \T $t[k] \gets 0$; coeff $\gets$ quad[branch\_id][$k$].coeff
\vsitem \T \xif coeff $\ne 0$ \xthen
\vsitem \T \T new\_$i \gets n \times $ quad[branch\_id][$k$].shift\_$i + i$; new\_$j \gets n \times $ quad[branch\_id][$k$].shift\_$j + j$
\vsitem \T \T $t[k] \gets$ coeff $\times$ \textsc{Compute-Input-Cell}($Z$, stage\_id, parent\_id, new\_$i$, new\_$j$, $2n$, height $-1$, quad)

\vsitem \xreturn $t[0] + t[1]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Output-Matrices}(Z, \text{stage\_id, root\_id, branch})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem height $\gets$ \#levels in the stage; \#leaves $\gets 7^{\text{height}}$ 

\vsitem \xparallelfor node $\gets 0$ \xto \#leaves $-1$ \xdo
\vsitem \T leaf\_id $\gets$ (root\_id $- 1$) $\times$ \#leaves $+ $ node 
\vsitem \T \xif last stage \xthen $Z$[stage\_id][leaf\_id][0,0] $\gets$ $U$[stage\_id][leaf\_id][0,0] $\times$ $V$[stage\_id][leaf\_id][0,0]
\vsitem \T \xelse \textsc{Compute-Output-Matrices}$(Z, \text{stage\_id + 1, leaf\_id, branch})$

\vsitem \xparallelfor $i \gets 0$ \xto $n-1$ \xdo \label{line:spawnoutputrows}
\vsitem \T \xparallelfor $j \gets 0$ \xto $n-1$ \xdo \label{line:spawnoutputcols}
\vsitem \T \T  \textsc{Compute-Output-Cell}($Z$, stage\_id, root\_id, $i, j, n$, height, branch)

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Output-Cell}(Z, \text{stage\_id, node\_id, $i, j, n$, height, branch})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem \xif height $= 0$ \xthen \xreturn $Z$[stage\_id + 1][node\_id][$i, j$]
\vsitem shift\_$i \gets [i > n/2]$; shift\_$j \gets [j > n/2]$ \xcomment{[ ] is the Iversion bracket}
\vsitem quad\_id $\gets 2 $ shift\_$i + $ shift\_$j$; new\_$i \gets i - (n/2) $ shift\_$i$; new\_$j \gets j - (n/2) $ shift\_$j$

\vsitem \xparallelfor $k \gets 0$ \xto $6$ \xdo
\vsitem \T $t[k] \gets 0$; coeff $\gets$ branch[quad\_id][$k$]
\vsitem \T \xif coeff $\ne 0$ \xthen
\vsitem \T \T child\_id $\gets$ (node\_id $- 1$) $\times 7 + k$
\vsitem \T \T $t[k] \gets$ coeff $\times$ \textsc{Compute-Output-Cell}($Z$, stage\_id, child\_id, new\_$i$, new\_$j$, $n/2$, height $- 1$, branch)
\vsitem \xreturn $\sum_{k = 0}^{6} t[k]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
}
\vgap{}
\caption{The \textsc{Strassen-S} MM algorithm.}
\label{fig:strassen-algorithm}
\end{figure*}


\begin{figure}
\begin{mycolorbox}{$\AlmostSort(n_c, n, l_0, d, m, B, C, D)$
\vspace{-.3cm}
\begin{align*}
n_c &\text{ : size of array to sort (only $B[l_0, ..., l_0 + n_c - 1]$ is occupied)} \hspace{2cm}~ \\
n &\text{ : size of the array at the highest level of recursion} \\
l_0 &\text{ : location where the array to sort begins} \\
d &\text{ : depth of current call in recursion tree} \\
m &\text{ : multiple of extra memory to use} \\
B[l_0, ..., l_0 + n_c m - 1] &\text{ : contains array to be sorted} \\
C[l_0, ..., l_0 + n_c m - 1] &\text{ : ancillary space} \\
D[l_0, ..., l_0 + n_c m - 1] &\text{ : where prefix sums will be stored (for indexing)}
\end{align*}
}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1em}

% ------ base case
\vsitem \xif $d \geq \log \log \log n$ \xdo  $\textsc{Cole-Ramachandran}(B[l_0, l_0 + n_c - 1])$ and \xreturn
\vsitem[] $\{ \text{ Partitioning $B$; choose $\sqrt{n_c} - 1$ pivots with oversampling factor $s$ } \}$ \dotfill
\vsitem $s \gets \log^3 n_c$
\vsitem $P \gets$ sample with repetition $(\sqrt{n_c} + 1) s$ elements from $B[l_0,...,l_0 + n_c - 1]$
\vsitem $P \gets \EpsilonWaySort(P, 1/2)$
\vsitem $P[0] \gets -\infty$; $P[(\sqrt{n_c} + 1) s] \gets +\infty$
\vsitem[] $\{ \text{ Nondeterministically partition $B$ into $C$ } \}$ \dotfill
\vsitem \xparallelfor $a \in B[l_0,...,l_0 + n_c - 1]$ \xdo
\vsitem \T Find some $i$ s.t. $P[i \cdot s] \leq a \leq P[(i+1) s]$ \label{line:implicit-binary-search}
\vsitem \T Choose a random number $j \in [0, ..., m \sqrt{n_c} - 1]$
\vsitem \T Attempt to assign $C[i m \sqrt{n_c} + j] \gets a$; in case of collision do nothing
% ------ cleaning up
\vsitem \xparallelfor $i \gets l_0$ \xto $l_0 + n_c - 1$ \xdo $B[i] \gets $ null
\vsitem[] $\{ \text{ Compact the partitions of $C$ into $B$ } \}$ \dotfill
\vsitem \xparallelfor $i \gets 0$ \xto $\sqrt{n_c} - 1$ \xdo
\vsitem \T lo $\gets l_0 + im\sqrt{n_c}$; hi $\gets l_0 + (i + 1)m\sqrt{n_c} - 1$
\vsitem \T $D[\text{lo}, ..., \text{hi}] \gets \textsc{Indicator-Prefix-Sum}(C[\text{lo}, ..., \text{hi}])$
\vsitem \T \xparallelfor $j \gets$ lo \xto hi \xdo
\vsitem \T \T $D[j] \gets D[j] + im\sqrt{n_c}$
\vsitem \xparallelfor $i \in [l_0,...,l_0 + n_c m - 1]$ \xdo
\vsitem \T \xif $C[i]$ is not null \xdo
\vsitem \T \T $B[D[i]] \gets C[i]$
\vsitem \T \T $C[i] \gets $ null
\vsitem[] $\{ \text{ Divide and Conquer } \}$ \dotfill
\vsitem \xparallelfor $i \gets 0$ \xto $\sqrt{n_c} - 1$ \xdo
\vsitem \T $\AlmostSort(\sqrt{n_c}, n, l_0 + im\sqrt{n_c}, d + 1, m, B, C, D)$
\vsitem[] $\{ \text{ Compact the final result } \}$ \dotfill
\vsitem $C \gets B$; $D \gets \textsc{Indicator-Prefix-Sum}(C)$
\vsitem \xparallelfor $i \gets 0$ \xto $n_c m - 1$ \xdo
\vsitem \T \xif $C[i]$ is not null \xthen
\vsitem \T \T $B[D[i]] \gets C[i]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\caption{Listing for the randomized sorting algorithm {\AlmostSort}. $\textsc{Boolean-Prefix-Sum}(A)$ is a standard prefix sum taken over the indicator function of $A$, i.e. the function which is 0 where $A[i]$ is null, and 1 elsewhere. Note that on line \ref{line:implicit-binary-search} we have an implicit binary search across $\sqrt{n_c}$ elements. } 
\label{fig:sorting-algorithm-almost}
\end{figure}

\begin{figure}
\centering
\scalebox{0.75}{
\begin{mycolorbox}{$\MainSort(A, n)$}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1em}

\vsitem[] $\{ \textbf{ Part 1:}\text{ Sorting the majority of $A$} \}$ \dotfill
\vsitem $m \gets \log n \log \log \log n / \log \log n$; Allocate arrays $B, C, D$ of size $n m$;  $B[0, ..., n-1] \gets A$
\vsitem $\AlmostSort(n, n, 0, 0, m, B, C, D)$
\vsitem num\_sorted $\gets $ smallest $i$ s.t. $B[i] =$ null
% ------ uniform memory; place all of (A - B) once
\vsitem[] $\{ \textbf{ Part 2:}\text{ Combining unsorted elements into $B$} \}$ \dotfill
\vsitem Set all elements of $C$ and $D$ to null
\vsitem Allocate arrays $E, F$ of size $n$
\vsitem[] $\{ \text{ Pass 1: Finding and indexing all nonempty buckets } \}$ \dotfill
\vsitem \xparallelfor $a \in A[0, ..., n-1]$ \xdo
\vsitem \T Find smallest $i$ s.t. $B[i] \leq a < B[i + 1]$
\vsitem \T \xif $a \neq B[i]$ \xthen
\vsitem \T \T Choose a random number $j \in [0, ..., m - 1]$
\vsitem \T \T Attempt to assign $C[i \cdot m + j] \gets a$; in case of collision do nothing
% ------ find all nonempty buckets and index them
\vsitem $D \gets \textsc{Indicator-Prefix-Sum}(C)$
\vsitem \xparallelfor $i \gets 0$ \xto $n$ \xdo
\vsitem \T \xif $D[i \cdot \text{block\_size}] \neq D[(i + 1) \cdot \text{block\_size} - 1]$ \xthen $E[i] = 1$
\vsitem $F \gets \textsc{Prefix-Sum}(E)$
% ------ clear our work space
\vsitem Set all elements of $C$ and $D$ to null
% ------ uniform memory to nonempty buckets; place all of (A - B) once
\vsitem[] $\{ \text{ Pass 2: Approximating the size of each bucket } \}$ \dotfill
\vsitem block\_size $\gets \log^3 n \log^2 \log \log n / \log^3 \log n$
\vsitem \xparallelfor $a \in A[0, ..., n-1]$ \xdo
\vsitem \T Find smallest $i$ s.t. $B[i] \leq a < B[i + 1]$
\vsitem \T \xif $a \neq B[i]$ \xand $E[i] = 1$ \xdo
\vsitem \T \T Choose a random number $j \in [0, ..., \text{block\_size} - 1]$
\vsitem \T \T Attempt to assign $C[(F[i] - 1) \cdot \text{block\_size} + j] \gets a$; in case of collision do nothing
% ------ generate running count approximation
\vsitem $D \gets \textsc{Indicator-Prefix-Sum}(C)$
\vsitem \xparallelfor $i \gets 0$ \xto num\_sorted $-\;1$ \xdo
\vsitem \T \xif $E[i] = 0$ \xthen $E[i] = 1$
\vsitem \T \xelse $E[i] = D[F[i] \cdot \text{block\_size} - 1] - D[(F[i] - 1) \cdot \text{block\_size}]$
\vsitem $F \gets \textsc{Prefix-Sum}(E)$
% ------ clear our work space
\vsitem clear $C$ and $D$
% ------ nonuniform memory; log n placements
\vsitem[] $\{ \text{ Pass 3: Sampling elements into their buckets with $\log n$ repetitions } \}$ \dotfill
\vsitem \xparallelfor $i \gets 0$ \xto $n - 1$ \xdo
\vsitem \T \xparallelfor $j \gets 0$ \xto $\log n - 1$ \xdo
\vsitem \T \T Choose a random number $k = H(j, (F[i] - E[i])m, F[i]m - 1)$ \label{line:hash-function}
\vsitem \T \T Attempt to assign $C[k] \gets a$; in case of collision do nothing
% ------ remove duplicates
\vsitem[] $\{ \text{ Removing duplicates and compacting } \}$ \dotfill
\vsitem chunk\_size $\gets n \log \log \log n / \log \log n$
\vsitem \xfor $i \gets 0$ to $n / \text{chunk\_size} - 1$
\vsitem \T \xparallelfor $a \in A[i \cdot \text{chunk\_size}, ..., (i + 1) \cdot \text{chunk\_size}-1]$ \xdo
\vsitem \T \T Find smallest $i$ s.t. $B[i] \leq a < B[i + 1]$
\vsitem \T \T \T $\textsc{Keep-Single}(C, a, n, H, (F[i] - E[i])m, F[i]m - 1)$ \label{line:keep-single}
\vsitem \xparallelfor $i \gets 0$ \xto num\_sorted $-\;1$ \xdo
\vsitem \T $D[(F[i] - E[i])m, ..., F[i]m - 1] \gets \textsc{Indicator-Prefix-Sum}(C[(F[i] - E[i])m, ..., F[i]m - 1])$
\vsitem \T \xparallelfor $j \gets (F[i] - E[i])m$ \xto $F[i]m - 1$ \xdo
\vsitem \T \T $D[j] \gets D[j] + (F[i] - E[i])m$
\vsitem \xparallelfor $i \gets 0$ \xto $n m-1$ \xdo
\vsitem \T \xif $C[i] \neq $ null \xthen $\{~ A[D[i]] \gets C[i]; C[i] \gets \text{null} ~\}$
\vsitem \xparallelfor $i \gets 0$ \xto num\_sorted $-\;1$ \xdo
\vsitem \T \text{lo} $\gets (F[i] - E[i])m$; \text{hi} $\gets \text{lo} + E[i] - 1$
\vsitem \T $A[\text{lo}, ..., \text{hi}] \gets \textsc{Cole-Ramachandran}(A[\text{lo}, ..., \text{hi}])$
\vsitem $D \gets \textsc{Indicator-Prefix-Sum}(A)$
\vsitem \xparallelfor $i \gets 0$ \xto $n m-1$ \xdo
\vsitem \T \xif $A[i] \neq $ null \xthen $\{~ C[D[i]] \gets A[i]; A[i] \gets \text{null} ~\}$
\vsitem $A \gets C$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
}
\caption{Listing for {\MainSort}. $H(i, \text{lo}, \text{hi})$ on line \ref{line:hash-function} is a hash function which maps the triple $(i, \text{lo}, \text{hi})$ to a single value in the range $[\text{lo}, ..., \text{hi}]$. $\textsc{Keep-Single}(A, a, n, H, \text{lo}, \text{hi})$ on line \ref{line:keep-single} is a function which performs a $\textsc{Prefix-Sum}$-like operation to index the instances of $a$ at the (assumed distinct) locations $H(i, \text{lo}, \text{hi})$ ($i = 0, ..., \log n - 1$), and then sets all but one of the instances to null. }
\label{fig:sorting-algorithm-main}
\end{figure}












\begin{figure}
\centering
\includegraphics[width=0.85\textwidth]{images/fft-rway.pdf}
\caption{The $n^{\phi}$-way FFT algorithm. Here, $r = n^{\phi}$.}
\label{fig:fft-kway-diagram}
\end{figure}

\begin{figure}
\begin{minipage}{0.48\textwidth}
\begin{mycolorbox}{$\textsc{FFT-sp}(x, \ell, n, i)$}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\algoinput Input array $x$, level $\ell$, size $n$, entry $i$
\algooutput DFT entry $y^{\ell}[i]$ 
\algomiddlespace

\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem \xif $n = 1$ \xthen \xreturn $x[0]$
\vsitem $j \gets i - (n/2) \times [i < n/2]$; $w \gets w_n^{-j}$
\vsitem \xpar $u \gets$ \textsc{FFT-sp}$(x,\ell + 1,n/2,j)$
\vsitem[] \xblankpar $v \gets $ \textsc{FFT-sp}$(x + 2^{\ell},\ell + 1,n/2,j)$
\vsitem \xreturn $u - wv \times (-1)^{[i < n/2]}$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\begin{minipage}{0.01\textwidth}
~
\end{minipage}
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{images/fft-sp-diagram.pdf}
\end{minipage}
\caption{Left: Single-point FFT algorithm to compute the $i$th entry of the DFT of $n$-sized array $x$. Symbol $[~]$ represents the Iversion bracket. Initial invocation is \textsc{FFT-sp}$(a, 1, n, i)$. Right: Single-point FFT evaluation of DFT entry $y^{\ell}[i]$ at level $\ell$ using the DFT entries $y^{\ell + 1}[i]$ of the child nodes at level $\ell + 1$. Note that $y^{\ell}[n/2+i]$ also depends on the $y^{\ell + 1}[i]$ entries.} 
\label{fig:fft-single-point-algorithm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{images/fft-stages}
\caption{Stages in the 2-way FFT algorithm with single-point computations.}
\label{fig:fft-stages-2way}
\end{figure}

\begin{figure*}
\centering
\begin{minipage}{\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{mycolorbox}{$\textsc{FFT-2way-stages}(y, a, n, \psi)$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem \xparallelfor $i \gets 0$ \xto $n - 1$ \xdo $y^{(0)}[i] \gets a[i]$

\vsitem \xfor stage $s \gets 1$ \xto $1/\psi$ \xdo
\vsitem \T $\ell_s \gets (1 - s\psi) \log n$ \xcomment level number
\vsitem \T \xparallelfor $j \gets 0$ \xto $2^{\ell_s} - 1$ \xdo
\vsitem \T \T \xparallelfor $i \gets 0$ \xto $n/2^{\ell_s} - 1$ \xdo
\vsitem \T \T \T $y^{(\ell_s)}[j + i \cdot 2^{\ell_s}] \gets$ 
\vsitem[] \T \T \T $\textsc{FFT-sp}(y^{(\ell_{(s-1)})} + j, \ell_s, n/2^{\ell_s}, i, {\ell}_{s - 1})$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{mycolorbox}{$\textsc{FFT-sp}(x, \ell, n, i, \ell')$}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\algoinput Input array $x$, level $\ell$, size $n$, entry $i$, stop at level $\ell'$
\algooutput DFT entry $y^{\ell}[i]$ 
\algomiddlespace

\noindent
\begin{enumerate}
\setlength{\itemindent}{-1.5em}

\vsitem \xif $\ell = \ell'$ \xthen \xreturn $x[i]$ \label{line:fft-sp-basecase}
\vsitem $j \gets i - (n/2) \times [i < n/2]$; $w \gets w_n^{-j}$
\vsitem \xpar $u \gets$ \textsc{FFT-sp}$(x,\ell + 1,n/2,j, \ell')$
\vsitem[] \xblankpar $v \gets $ \textsc{FFT-sp}$(x + 2^{\ell},\ell + 1,n/2,j, \ell')$
\vsitem \xreturn $u - wv \times (-1)^{[i < n/2]}$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\caption{The 2-way \textsc{FFT} algorithm with stages.}
\label{fig:fft-2way-stages}
\end{minipage}
\end{figure*}




==> mm-bound.tex <==
\subsection{Proof of Theorem \ref{thm:strassen-lower-bound}}
\label{ssec:strassen-lower-bound}
In this section, we give lower bounds of span and work for matrix multiplication (MM) parallel algorithms that perform $\Th{n^w}$ serial work. 

We consider the binary-forking model without atomics~\cite{BlellochFiGuSu2019}. In this model, every binary operation (addition, subtraction, multiplication and division) is associated with a memory location. Specifically, the output of such binary operation needs to be written to a memory location. Concurrent reads from a memory location are allowed, while concurrent writes are not.

Let $A$ be a matrix multiplication serial algorithm with $\Th{n^w}$ work where $w \ge 2$. Let $T_{\infty}(n, w, s)$ denote the span of any parallel algorithm $B$ that parallelize the serial algorithm $A$ using $s$ units of space. We do not make any restriction on the number of processors used. We remark that only heap space is counted in $s$ (all our previous algorithms also allocate space from heap memory). 

We get the first lower bound as follows. When we use $s$ units of memory locations, then from the pigeonhole principle, there must exist a memory location that is subjected to $\Th{n^w/s}$ write operations. As concurrent writes to a memory location are not allowed, the following lower bound holds: $T_{\infty}(n, w, s) = \Om{n^w/s}.$

We get the second lower bound from a more general PRAM CREW model. Thus, it holds for a more restricted binary-forking model. When we have an unbounded \#memory locations and unbounded \#processors, the following lower bound ~\cite{jaja1997introduction} holds for the computation of $x_1+x_2+\cdots + x_n$ (array-sum) where every $s_i\in \{0,1\}$: $T_{\infty}(n, w, \infty) = \Om{\log n}.$

As matrix multiplication is at least as hard as array-sum, it must have $\Omega(\log n)$ span. Combining both the lower bounds, we get the following: $T_{\infty}(n, w, s) = \Om{\max(n^w / s, \log n)}.$

==> mm-conc.tex <==
\section{Conclusion}
\label{ref:conclusion}

There is a trade-off between space, parallelism, and communication complexity of algorithms on shared-memory machines. This paper presented a hybrid static 2.5-D rectangular matrix multiplication algorithm that given a fixed amount of space can be used to simultaneously achieve high parallelism and good cache performance. The paper also presented two efficient hybrid tensor contraction algorithms that have space-parallelism-locality trade-off. We believe that it is possible to develop a generic theory to design shared-memory hybrid algorithms having space-parallelism-locality trade-off for different classes of problems.

==> mm-lim-tens.tex <==
\subsection{Tensor Contraction Algorithm}
\label{subsec:tc}
A $d$-dimensional \highlight{tensor}, for $d \ge 1$, denoted by $T(i_1, \allowbreak .., \allowbreak i_d)$, where $i_j \in [1, n_j]$ for $j \in [1, d]$, is an $n_d$-sized array of $(d - 1)$-D tensors $T_j(i_1, \allowbreak .., \allowbreak i_{d - 1})$ for $j \in [1, n_d]$. $T(i_1,.., i_d) = [T_1(i_1,.., i_{d - 1}) ~T_2(i_1,.., i_{d - 1}) ~\cdots ~T_{n_d}(i_1,.., i_{d - 1})]$. The number of indices $d$ of a tensor is also called rank, order, or degree of the tensor. A $d$-D tensor can be represented by a $d$-D matrix. A $0$-D tensor is a number.

Let $T\{i_1, \allowbreak .., i_a\}$ denote a tensor $T$ with any arrangement of indices $\{i_1, \allowbreak .., i_a\}$. \highlight{Tensor contraction} between an $(a + c)$-order tensor $A\{ i_1,\allowbreak ..,\allowbreak i_a,\allowbreak k_1,\allowbreak ..,\allowbreak k_c \}$ and a $(b+c)$-order tensor $B\{ j_1,\allowbreak ..,\allowbreak j_b,\allowbreak k_1,\allowbreak ..,\allowbreak k_c \}$, denoted by $A \otimes B$, is defined as an $(a+b)$-order tensor $C[ i_1,\allowbreak ..,\allowbreak i_a,\allowbreak j_1,\allowbreak ..,\allowbreak j_b ]$. We assume that $i_{\ell} \in [1, m_{\ell}]$, $j_{\ell} \in [1, n_{\ell}]$, and $k_{\ell} \in [1, q_{\ell}]$ for all feasible values of $\ell$. We say that the $c$ indices $\{k_1, \allowbreak .., k_c\}$ are \textit{contracted} and the $(a + b)$ indices $\{ i_1,\allowbreak ..,\allowbreak i_a,\allowbreak j_1,\allowbreak ..,\allowbreak j_b \}$ are \textit{uncontracted}. Tensor contraction can be mathematically defined as $C[i_1,\allowbreak ..,\allowbreak i_a,\allowbreak j_1,\allowbreak ..,\allowbreak j_b] = \sum_{k_1} \cdots \sum_{k_c} ( A\{ i_1,\allowbreak ..,\allowbreak i_a,\allowbreak k_1,\allowbreak ..,\allowbreak k_c \} \times B\{ j_1,\allowbreak ..,\allowbreak j_b,\allowbreak k_1,\allowbreak ..,\allowbreak k_c \} )$ and can be regarded as a generalization of matrix multiplication. A few examples of the problem are: $(i)$ $(c = 2)$ $A(i_1, k_1, i_2, k_2) \otimes B(k_1, j_1, k_2, j_2) = C(i_1, i_2, j_1, j_2)$, $(ii)$ $(c = 2)$ $A(k_1, k_2) \otimes B(k_1, k_2) = C()$, $(iii)$ $(c = 1)$ $A(i, k) \otimes B(k, j) = C(i, j)$, $(iv)$ $(c = 0)$ $A(i_1, i_2) \otimes B(j_1, j_2) = C(i_1, i_2, j_1, j_2)$, and $(v)$ $(c = 0)$ $A(i_1) \otimes B(j_1, j_2, j_3, j_4) = C(i_1, j_1, j_2, j_3, j_4)$.

The example with $c = 1$ is an instance of matrix multiplication where a single dimension gets contracted. The examples with $c = 2$ are instances of tensor contraction where two common indices between tensors $A$ and $B$ get contracted. The examples with $c = 0$ do not lead to contraction. Note that the order of the tensor product can be greater than, smaller than, or equal to the orders of the input tensors. 

\begin{figure*}
\centering
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{TC-MM-OPT}(X,U,V)$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\vspace{0.1cm}
\algorequire $x \ge 1$
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem $\textsc{TT}(U',U, n, u+x)$ \xcomment{$U' \gets $ Transpose of tensor $U$}
\vsitem $\textsc{TT}(V',V, n, x+v)$ \xcomment{$V' \gets $ Transpose of tensor $V$}
\vsitem $\textsc{TF}(A,U', u, x)$ \xcomment{$A \gets $ Flatten tensor $U'$ to matrix}
\vsitem $\textsc{TF}(B,V', x, v)$
\xcomment{$B \gets $ Flatten tensor $V'$ to matrix}
\vsitem $\textsc{RMM-OPT}(C_{n^{u} \times n^{v}}, A_{n^{u} \times n^{x}}, B_{n^{x} \times n^{v}})$ \xcomment $C \gets A \times B$
\vsitem $\textsc{TD}(X, C, u, v)$
\xcomment{$X \gets$ Deflatten matrix $C$ to tensor}

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{TT}(W,R,n,d)$ \xcomment Tensor Transposition}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem \xif $n = 1$ \xthen $W \gets R$; \xreturn
\vsitem $[r_1, \ldots, r_d] \gets$ rank vector (ranks of the indices of $R$ in the transposed tensor $W$) 
\vsitem \xparallelfor $p_1 \leftarrow 1$ \xto $2$ \xdo
\vsitem $\cdots$
\vsitem \xparallelfor $p_d \leftarrow 1$ \xto $2$ \xdo
\vsitem \T $\textsc{TT}(W_{p_1,..,p_d}, R_{p_{r_1},..,p_{r_d}}, n/2, d)$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{TF}(M,T,s', s'')$ \xcomment Tensor Flattening}
\begin{minipage}{0.99\textwidth}
{\codesize

\algotopspace{}
\noindent 
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem \xif $n = 1$ \xthen $M \gets T$; \xreturn
\vsitem \xparallelfor $i_1 \leftarrow 1$ \xto $2$ \xdo
\vsitem $\cdots$
\vsitem \xparallelfor $i_{s'} \leftarrow 1$ \xto $2$ \xdo
\vsitem \T \xparallelfor $j_1 \leftarrow 1$ \xto $2$ \xdo
\vsitem \T $\cdots$
\vsitem \T \xparallelfor $j_{s''} \leftarrow 1$ \xto $2$ \xdo
\vsitem \T \T $I \gets \textsc{Linearize}(i_1, \ldots, i_{s'})$; $J \gets \textsc{Linearize}(j_1, \ldots, j_{s''})$  \xcomment $I \in [1, 2^{s'}]$, $J \in [1, 2^{s''}]$
\vsitem \T \T $\textsc{TF}(M_{I,J}, T_{i_1, ..,i_{s'},j_1,..,j_{s''}}, s', s'')$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{\textsc{RMM-OPT}$(X^{[0 .. r - 1]}_{a \times c}, U_{a \times b}, V_{b \times c})$ \xcomment Hybrid static 2.5-D}
\begin{minipage}{0.99\textwidth}
{\codesize
\vspace{-0.25cm}
\algorequire $\Th{rac}$ space, $rac$ processors

\noindent 
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem Allocate $r \in [1, b]$ planes $X^{[0 .. r - 1]}$ all at once
\vsitem \textsc{RMM-OPT$'$}$(X^{[0 .. r - 1]}, U, V)$ \xcomment Uses $r \in [1, b]$ planes
\vsitem \textsc{MM-ReduceR}$(X^{[0..r - 1]}, a, c)$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{\textsc{RMM-OPT$'$}$(X^{[\ell .. h]}_{a \times c}, U_{a \times b}, V_{b \times c})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent 
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif $\ell = h$ \xthen $\textsc{RMM}(X^{[\ell]}, U, V)$ \xcomment Single plane
\vsitem \xelse \xcomment Multiple planes

\vsitem \T \xif $a \ge \max(b, c)$ \xthen
\vsitem \T \T \xpar \textsc{RMM-OPT$'$}$(X_{T}^{[\ell .. h]}, U_{T}, V)$, \textsc{RMM-OPT$'$}$(X_{B}^{[\ell .. h]}, U_{B}, V)$ 
\vsitem \T \xelseif $b \ge \max(a, c)$ \xthen
\vsitem \T \T $m \gets (\ell + h) / 2$
\vsitem \T \T \xpar \textsc{RMM-OPT$'$}$(X^{[\ell .. m]}, U_{L}, V_{T})$, \textsc{RMM-OPT$'$}$(X^{[m+1 .. h]}, U_{R}, V_{B})$
\vsitem \T \xelseif $c \ge \max(a, b)$ \xthen
\vsitem \T \T \xpar \textsc{RMM-OPT$'$}$(X_{L}^{[\ell .. h]}, U, V_{L})$, \textsc{RMM-OPT$'$}$(X_{R}^{[\ell .. h]}, U, V_{R})$
\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\vspace{-0.4cm}
\caption{The \textsc{TC-MM-OPT} algorithm.}
\label{fig:tensor-contraction}
\vspace{-0.2cm}
\end{figure*}

\hide{
\begin{figure}
\begin{center}
\begin{minipage}{0.99\textwidth}
\hspace{-0.1cm}
\includegraphics[width=0.255\textwidth]{tc_forkjoin.pdf}
\hspace{-0.4cm}
\includegraphics[width=0.255\textwidth]{tc_continuous.pdf}
\end{minipage}
\caption{Left and right: \textsc{TC} algorithm using and not using fork-join parallel computation model, respectively.}
\label{fig:tensor-contraction-diagrams}
\end{center}
\end{figure}
}

For simplicity, we consider \highlight{hypercube tensors} i.e., tensors in which the sizes of all dimensions are the same and are equal to, say, $n$. A parallel, not cache-efficient iterative algorithm \textsc{TC\text{-}Loop} to compute tensor contraction is shown in Figure \ref{fig:tensor-contraction}. We use the symbols $U, V, X$ instead of $A, B, C$, respectively, to maintain consistency of the algorithmic notations used in the paper.\\  



%----------------
\para{\textsc{TC-MM-OPT}: Hybrid Tensor Contraction using 2.5-D Matrix Multiplication}
It is possible to solve the tensor contraction problem by transforming it to the matrix multiplication problem. Figure \ref{fig:tensor-contraction} gives a hybrid tensor contraction algorithm \textsc{TC-MM-OPT} that uses a rectangular hybrid static 2.5-D matrix multiplication algorithm \textsc{MM-OPT}. We explain the working of the algorithm using an example. 

\vspace{0.1cm}
\noindent
\textit{Tensor Transposition.} Suppose we want to compute the tensor contraction of $U(i_1, k_1, i_2, k_2)$ and $V(j_1, j_2, k_2, k_1)$. We invoke $\textsc{TC-MM-OPT}$ to read from $U$ and $V$. The first step in the algorithm is to obtain a proper ordering of the indices by invoking the tensor transposition algorithm $\textsc{TT}$.  The indices of tensor $U$ are partitioned in such a way that all uncontracted (resp. contracted) indices are to the left (resp. right) of the partition. Similarly, the indices of tensor $V$ are partitioned in such a way that all uncontracted (resp. contracted) indices are to the right (resp. left) of the partition. For our example, $U(i_1, k_1, i_2, k_2)$ is transposed to $U'(i_1, i_2, k_1, k_2)$ using the \textit{rank vector} $[1, 3, 2, 4]$ because the second (resp. third) index of $U$ is mapped to the third (resp. second) index of $U'$. Similarly, the tensor $V(j_1, j_2, k_2, k_1)$ is transposed to $V'(k_1, k_2, j_1, j_2)$ using the rank vector $[3, 4, 2, 1]$.

We could have transposed a tensor using a simple iterative algorithm. However, the iterative algorithm would not have exploited the spatial locality. The \textsc{TT} algorithm uses recursive divide-and-conquer to exploit spatial data locality and hence has optimal cache performance. The recursive divide-and-conquer matrix transpose from \cite{FrigoLePrRa1999} is a special case of the \textsc{TT} algorithm. The working of the algorithm is as follows. Suppose we want to transpose a $d$-D hypercubic tensor $T(\ell_1, \ldots, \ell_d)$ to $T'(\ell_{r_1}, \ldots, \ell_{r_d})$, then $[r_1, \ldots, r_d]$ is the rank vector, where $[r_1, \ldots, r_d]$ is a permutation of $[1, \ldots, n]$. We split $T$ into $2^{d}$ orthants $T_{p_1 \ldots p_d}$ for all values $p_i \in [1, 2]$, $i \in [1, d]$. Then, the orthant $T_{p_1 \ldots p_d}$ gets transposed to $T'_{p_{r_1} \ldots p_{r_d}}$. As an example, consider the transpose of $T(\ell_1, \ell_2, \ell_3, \ell_4, \ell_5)$ to $T(\ell_2, \ell_1, \ell_5, \ell_4, \ell_3)$ for all feasible values of the indices. The rank vector is $[2,1,5,4,3]$. As there are five dimensions, there will be $2^5$ orthants. The orthant $T_{11221}$ (i.e., $p_1 = 1, p_2 = 1, p_3 = 2, p_4 = 2, p_5 = 1$) will get transposed to $T'_{11122}$ (i.e., $p_2 = 1, p_1 = 1, p_5 = 1, p_4 = 2, p_3 = 2$). Now, this idea is applied recursively to obtain the tensor transposition.

\vspace{0.1cm}
\noindent
\textit{Tensor Flattening.} We convert the input tensors to matrices because we can use a cache-efficient MM algorithm to solve the tensor contraction problem. In our original example, after tensor transposition, we obtain $U'(i_1, i_2, k_1, k_2)$ and $V'(k_1, k_2, j_1, j_2)$. We flatten tensor $U'$ (resp. $V'$) to matrix $A$ (resp. $B$) using the tensor flattening algorithm \textsc{TF}. The tensor flattening algorithm transforms an $(s + s')$-D tensor $T$ to a matrix $M$ such that an element of $T$ uniquely maps to an element of $M$. Specifically, the element $T[i_1, \ldots, i_s, j_1, \ldots, j_{s'}]$ maps to $M[I, J]$ such that $(i_1, \ldots, i_s)$ dimensions are linearized to $I$ and $(j_1, \ldots, j_{s'})$ dimensions are linearized to $J$. Using the algorithm, we transform $U'(i_1, i_2, k_1, k_2)$ to $A(I, K)$, where $I$ represents the linearization of the uncontracted dimensions and $J$ represents the linearization of the contracted dimensions of the tensor $U'$. Similarly, we transform $V'(k_1, k_2, j_1, j_2)$ to $B(K, J)$. The obtained matrices $A$ and $B$ are rectangular matrices of sizes $n^u \times n^x$ and $n^x \times n^v$, respectively.

The tensor flattening algorithm \textsc{TF} works as follows. \textsc{TF} uses recursive divide-and-conquer similar to \textsc{TT} to exploit spatial data locality and hence it achieves optimal cache performance. Suppose we want to transpose a $(s' + s'')$-D hypercubic tensor $T$ to matrix $M$. We split $T$ into $2^{s' + s''}$ orthants and $M$ into $2^{s'} \times 2^{s''}$ submatrices. We flatten the orthant $T_{i_1, .., i_{s'}, j_1, .., j_{s''}}$ to submatrix $M_{I, J}$ such that $I$ is a linearization of $(i_1, \ldots, i_{s'})$ and $J$ is a linearization of $(j_1, \ldots, j_{s''})$. 

\vspace{0.1cm}
\noindent
\textit{2.5-D Rectangular Matrix Multiplication.} We use the 2.5-D hybrid static rectangular matrix multiplication algorithm \textsc{RMM-OPT} on matrices $A$ and $B$ to obtain the resulting matrix $C$ of size $n^u \times n^v$. \textsc{RMM-OPT} combines ideas from the rectangular MM algorithm presented in \cite{FrigoLePrRa1999} and \textsc{MM-OPT} described in Section \ref{sec:mm} for square MM. The working of \textsc{RMM-OPT} is very similar to that of \textsc{MM-OPT} in that if two child functions write to the same region, then we divide the total planes available $[\ell \ldots h]$ into two almost-equal groups $[\ell \ldots m]$ and $[m+1 \ldots h]$ and distribute them to the two child functions. For our example, we obtain $C(I, J)$ by multiplying $A(I, K)$ and $B(K, J)$.

\vspace{0.1cm}
\noindent
\textit{Tensor Deflattening.} We deflatten the obtained matrix to a tensor following the tensor deflattening algorithm \textsc{TD} that is similar but reverse of the tensor flattening algorithm. Using this process, we transform matrix $C$ of size $n^u \times n^v$ to tensor $X$ with $(i_1, \ldots, i_u, j_1, \ldots, j_v)$ dimensions. For our example, we deflatten matrix $C(I, J)$ to $X(i_1, i_2, j_1, j_2)$ and this is the final tensor product we wanted to compute.

\begin{theorem}
\label{thm:tc-opt}
\textsc{TC-OPT} has a complexity of $T_1(n) = \Oh{n^w}$, and $T_{\infty}(n)=\Th{n^x/r + w \log n + \log r}$.
\end{theorem}

==> mm-lim.tex <==
\section{Optimal Parallelism with Space Constraints}
\label{sec:limited-space}

\subsection{Classical Matrix Multiplication Algorithms}
The straightforward triply-nested loop MM algorithm that uses $n^2$ parallel inner products uses reduction. This reduction that reduces an array sum uses $\Oh{n}$ extra space to achieve $\Oh{\log n}$ span. So, this straightforward looping MM algorithm in the binary forking model uses $\Oh{n^3}$ space to achieve a span of $\Oh{\log n}$.

\section{Matrix Multiplication (MM)}
\label{sec:mm}
The classic cubic computation square matrix multiplication problem is defined as follows. Given two $n \times n$ matrices $A$ and $B$ containing numbers stored in row-/column-major orders, the matrix product $C = A \times B$ is computed using the expression $C[i,j] = \sum_{k=1}^{n} A[i,k] \times B[k,j]$ for $i,j \in [1, n]$. 

\begin{figure*}
\begin{minipage}{\textwidth}
\hide{
\begin{mycolorbox}{\textsc{MM}$(X, U, V)$ \xcomment In-place 2-D}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif $X$ is a small matrix \xthen $\textsc{MM\textrm{-}Loop}(X, U, V)$
\vsitem \xelse
\vsitem \T \xpar \textsc{MM}$(X_{11}, U_{11}, V_{11})$, \textsc{MM}$(X_{12}, U_{11}, V_{12})$, \textsc{MM}$(X_{21}, U_{21}, V_{11})$, \textsc{MM}$(X_{22}, U_{21}, V_{12})$
\vsitem \T \xpar \textsc{MM}$(X_{11}, U_{12}, V_{21})$, \textsc{MM}$(X_{12}, U_{12}, V_{22})$, \textsc{MM}$(X_{21}, U_{22}, V_{21})$, \textsc{MM}$(X_{22}, U_{22}, V_{22})$					
\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
}
\begin{mycolorbox}{\textsc{MM-OPT}$(X^{[0 .. r - 1]}, U, V)$ \xcomment Hybrid static 2.5-D}
\begin{minipage}{0.99\textwidth}
{\codesize
\vspace{-0.25cm}
\algorequire $\Th{rn^2}$ space, $rn^2$ processors

\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem Allocate $r \in [1, n]$ planes $X^{[0 .. r - 1]}$ all at once
\vsitem \textsc{MM-OPT$'$}$(X^{[0 .. r - 1]}, U, V)$ 
\vsitem \textsc{MM-ReduceR}$(X^{[0..r - 1]}, n, n)$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{\textsc{MM-OPT$'$}$(X^{[\ell .. h]}, U, V)$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif $\ell = h$ \xthen $\textsc{MM}(X^{[\ell]}, U, V)$ \xcomment Single plane
\vsitem \xelse \xcomment Multiple planes
\vsitem \T $m \gets ( \ell + h ) / 2$
\vsitem \T \xpar \textsc{MM-OPT$'$}$(X_{11}^{[\ell .. m]}, U_{11}, V_{11})$, \textsc{MM-OPT$'$}$(X_{12}^{[\ell .. m]}, U_{11}, V_{12})$
\vsitem[] \xblankpar \textsc{MM-OPT$'$}$(X_{21}^{[\ell .. m]}, U_{21}, V_{11})$, \textsc{MM-OPT$'$}$(X_{22}^{[\ell .. m]}, U_{21}, V_{12})$
\vsitem[] \xblankpar \textsc{MM-OPT$'$}$(X_{11}^{[m + 1 .. h]}, U_{12}, V_{21})$, \textsc{MM-OPT$'$}$(X_{12}^{[m + 1 .. h]}, U_{12}, V_{22})$
\vsitem[] \xblankpar \textsc{MM-OPT$'$}$(X_{21}^{[m + 1 .. h]}, U_{22}, V_{21})$, \textsc{MM-OPT$'$}$(X_{22}^{[m + 1 .. h]}, U_{22}, V_{22})$						
\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vspace{-0.2cm}
\begin{mycolorbox}{\textsc{MM-ReduceR}$(X^{[0..r - 1]}_{a \times b}, a, b)$ \xcomment $X^{[0]} \gets X^{[0]} + \cdots + X^{[r - 1]}$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xparallelfor $i \gets 1$ \xto $a$ \xdo 
\vsitem \T \xparallelfor $J \gets 1$ \xto $\ceil{b/B}$ \xdo \xcomment $B =$ data block size
\vsitem \T \T local \xreducer $sum[1..B]$ data block
\vsitem \T \T \xrfor $k \gets 0$ \xto $r - 1$ \xdo $sum[1..B] \gets sum[1..B] + X^{[k]}[i, J\text{th data block}]$
\vsitem \T \T $X^{[0]}[i, J\text{th data block}] \gets sum[1..B]$ 

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\vspace{-0.3cm}
\caption{The \textsc{MM-OPT} algorithm. The algorithms are invoked with $U = A$, $V = B$, and $X$ being the total space available for the computation.}
\label{fig:matrixmultiplication}
\end{figure*}


Suppose we have total space and \#processors in the range $[n^2, n^3]$, say, $rn^2$, where $r \in [1, n]$, then we need an efficient MM algorithm that can make use of the extra memory and processors. So, we design the \textsc{MM-OPT} algorithm.\\

\hide{
\begin{corollary}[\highlighttitle{Cache-optimal MM-HD}]
\label{cor:mm-opt}
Suppose the total space used by the \textsc{MM-HD} algorithm is $rn^2$. Then, the upper bound on the number of processors that can be used such that the parallel algorithm remains cache-optimal is \begin{equation}
p = \Oh{\frac{n^3 (1 + B/\sqrt{M})+(n^2+n)\sqrt{M}}{M\sqrt{M} ( \log r \cdot \log (n^2/r) + n/r ) }}
\end{equation}
\end{corollary}
\begin{proof}
The parallel cache complexity on a $p$-processor machine with many private caches using a randomized work-stealing scheduler is $Q_{p}(n) = \Oh{Q_1(n) + p (M/B)T_{\infty}(n)}$ w.h.p. To achieve parallel cache-optimality, we must have $Q_p(n) = \Oh{Q_1(n)}$, which implies that $p = \Oh{Q_1(n) B / (T_{\infty}(n) M)}.$

From Theorem \ref{thm:mm-hd}, $Q_1(n) = \Oh{n^3/(B \sqrt{M}) + n^3/M + n^2/B + n}$ and $T_{\infty}(n) = \Th{\log r \cdot \log (n^2/r) + n/r}$. Substituting the values of $Q_1(n)$ and $T_{\infty}(n)$ in the equation for $p$, we obtain the desired result.
\end{proof}
}

\para{MM-OPT: Hybrid Static 2.5-D Algorithm} We present \textsc{MM-OPT} -- an algorithm for matrix multiplication that provides a trade-off between parallelism and cache locality parameterized by space. This is the first matrix multiplication algorithm to achieve the theoretically optimal span for any given amount of space in the binary forking model. The algorithm achieves the optimal cache complexity for a range of space at one end of the trade-off spectrum and the optimal $\Oh{\log n}$ span at the other end.

Figure \ref{fig:matrixmultiplication} shows the \textsc{MM-OPT} algorithm with static memory allocation. Suppose $r$ planes $X^{[0..r-1]}$ and $rn^2$ \#processors are available. Then, we can use the available space and processors to improve the parallel running time over that of \textsc{MM}. We can imagine as if $r$ space and $r$ processors are available to compute each cell of the output matrix. 

\textsc{MM-OPT} works as follows. Initially, we allocate $r$ planes all at once statically before invoking \textsc{MM-OPT$'$}. \hide{We could either allocate space by using global variables or by using static variables in the main function.}Then, we call \textsc{MM-OPT$'$} that uses all $rn^2$ processors to compute the matrix product storing partial sums in the $r$ planes $X^{[0..r-1]}$. Finally, we use the parallel reduction function \textsc{MM-ReduceR} on the $r$ planes that computes $X^{[0]} + \cdots + X^{[r - 1]}$ and stores the result in the zeroth plane $X^{[0]}$.

\hide{
The major difference between \textsc{MM-HD} and \textsc{MM-OPT} is as follows. In \textsc{MM-HD}, the extra memory allocation and sum-reduction happens inside the divide-and-conquer function \textsc{MM-HD$'$}. In contrast, in \textsc{MM-OPT}, the extra memory allocation and the reduction occurs outside the divide-and-conquer function \textsc{MM-OPT$'$}. Due to the separation of computation and reduction phases, the span of \textsc{MM-OPT} improves compared to that of \textsc{MM-HD}.
}

\begin{theorem}[\highlighttitle{MM-OPT: Hybrid static 2.5-D}]
\label{thm:MM-OPT} MM-OPT has a complexity of $T_1(n) = \Th{n^3}$, $T_{\infty}(n)=\Th{n/r + \log n + B}$ and $S_{\infty}(n) = \Th{r n^2}$. Let $f = (rn^2/M)^{1/3}$. Then $Q_1(n) = \mathcal{O}( (n^3 / (B \sqrt{M}) + n^3 / M + r n^2 / B + r^2 n)$ if $f > r$, and $Q_1(n) = \Oh{ rn^2 / B + f ( nr + f^2 ) }$, if $f \le r$.
\end{theorem}
\begin{proof} \textsc{MM-OPT} calls two functions: \textsc{MM-OPT$'$} and \textsc{MM-ReduceR}. The work, span, and space complexity of \textsc{MM-OPT$'$} dominates the corresponding complexity of \textsc{MM-ReduceR}. We assume that $r$ is a power of 2 for simplicity.  The analysis of work, span, and serial cache complexity of $\textsc{MM-OPT$'$}$ is as follows: $T_1'(n, r) = \Th{n^3}$ if $r = 1$ and $T_1'(n, r) = 8 T_1'(n/2, r/2) + \Th{1}$ if $r>1$.

{\small
\begin{tabular}{l l}
$T_{\infty}'(n, r) = \begin{cases} \Th{n} &\mbox{if } r = 1,\\ 
T_{\infty}'(n/2, r/2) + \Th{1}  & \mbox{if } r > 1. \end{cases}$ & $Q_1'(n, r) = \begin{cases} Q_1^{A}(n, r) &\mbox{if } r < n/\sqrt{M}, \\ 
Q_1^{B}(n, r)  & \mbox{if } r \ge n/\sqrt{M}. \end{cases}$\\
$Q_1^{A}(n, r) = \begin{cases} \Oh{n^3 / (B\sqrt{M}) + n^3 / M + n^2 / B + n} &\mbox{if } r = 1, \\ 
8 Q_1^{A}(n/2, r/2) + \Oh{1}  & \mbox{if } r > 1. \end{cases}$ & $Q_1^{B}(n, r) = \begin{cases} \Oh{rn^2 / B + rn} &\mbox{if } r n^2 \le \alpha M, \\ 
8 Q_1^{B}(n/2, r/2) + \Oh{1}  & \mbox{if } rn^2 > \alpha M.\end{cases}$ \\
\end{tabular}
}

We compute $Q_1'$ using two cases: $[$Case $A.]$ In this case, a subproblem switches to the in-place algorithm before fitting in the cache i.e, $(n/r)^2 > M$ or $r < n/\sqrt{M}$. Recurrence $Q_1^{A}$ models this case. We obtain $Q_1^{A}(n, r) = \mathcal{O}(n^3/(B \sqrt{M}) + n^3/M + rn^2/B + r^2n)$. $[$Case $B.]$ In this case, a subproblem fits in the cache before switching to the in-place algorithm i.e, $(n/r)^2 \le M$ or $r \ge n/\sqrt{M}$. Recurrence $Q_1^{B}$ models this case. We get $Q_1^{B}(n, r) = \Oh{rn^2/B + rn^2/M + r^{4/3}n^{5/3}/M^{1/3}}$.

$T_{1}^{''}(n,r)$, $T_{\infty}^{''}(n,r)$, and $Q_1^{''}(n,r)$ for \textsc{MM-ReduceR} are $\Th{rn^2}$, $\Th{\log n + B}$ and $\Th{rn^2/B + rn}$, respectively. So, solving the equations $T_{\infty}(n) = T_{\infty}^{'}(n,r) + T_{\infty}^{''}(n,r)$ and $Q_1(n) = Q_1^{'}(n,r) + Q_1^{''}(n,r)$ provide the desired results. \textsc{MM-ReduceR} is cache-aware as a result of exploiting optimal spatial locality from the algorithm.
\end{proof}

\hide{
Theorem \ref{thm:MM-OPT} tells us that the \textsc{MM-OPT} algorithm may not be cache-efficient depending on the value of $r$. When we choose large $r$, there will be more parallelism, but at the same time the parallel cache complexity will be worse.
}

\input{mm-lim-tens.tex}







==> mm-sort.tex <==
\section{$n^{\epsilon}$-way Merge Sort}
In this section, we present a simple merge-based parallel sorting algorithm parameterized on a fixed constant $\epsilon \in (0, 1]$, which achieves the optimal span of $\Oh{(1/\epsilon) \log n}$ but performs suboptimal work of $\Oh{(1/\epsilon) n^{1 + \epsilon}}$. We call this algorithm $n^{\epsilon}$-way merge sort.

Figure \ref{fig:multiway-sort} gives a pseudocode of the sorting algorithm. Choose a fixed constant $\epsilon \in (0, 1]$ such that $1/\epsilon$ is a natural number and suppose that $r = n^{\epsilon}$. The core idea of the algorithm is as follows. The input array $A[1..n]$ is split into $r$ subarrays, each having $n/r$ elements. All $r$ subarrays are sorted recursively. These subarrays are then merged using an $r$-way merger.  The working of the $r$-way merger consists of two stages. In the first stage, we compute $rank_i[k, j]$ in parallel, for all feasible values of $i,j,k$. The term $rank_i[k, j]$ represents the rank/position of $A_i[k]$ (the $k$th element of subarray $A_i$) in the merged list of $A_i$ and $A_j$. In the second stage, we compute $rank_i[k]$ in parallel, for all feasible values of $i,k$ using a reduction. The term $rank_i[k]$ represents the rank/position of $A_i[k]$ (the $k$th element of subarray $A_i$) in the merged list of the $r$ subarrays $A_1,A_2,\ldots, A_r$.

\begin{figure*}
\centering
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{Sort}(A, n, \epsilon)$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\vspace{0.1cm}
\algorequire $1/\epsilon$ is a natural number
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}
\vsitem \xif $\epsilon = 1$ \xthen  \textsc{Counting-Sort}$(A, n)$
\vsitem \xelse
\vsitem \T $r \gets n^{\epsilon}$; Split $A[1 .. n]$ into $r$ segments $A_1, A_2, \ldots, A_r$, each of size $n/r$
\vsitem \T \xparallelfor $k \gets 1$ \xto $r$ \xdo $\textsc{Sort}(A_k, n/r, \epsilon/(1 - \epsilon))$

\vsitem \T $A \gets$ \textsc{Merge}$(A_1, A_2, \ldots, A_r)$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Merge}(A_1, A_2, \ldots, A_r)$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}


\vsitem \xparallelfor $i \gets 1$ \xto $r$ \xdo
\vsitem \T \xparallelfor $j \gets i + 1$ \xto $r$ \xdo
\vsitem \T \T Merge $A_i$ and $A_j$ in $\Oh{n}$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\vspace{-0.4cm}
\caption{The \textsc{Sort} algorithm.}
\label{fig:multiway-sort}
\vspace{-0.2cm}
\end{figure*}































\begin{figure*}
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{Compute-Output-Arrays}(y, \text{stage\_id, root\_id})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem height $\gets$ \#levels in the stage; \#leaves $\gets 2^{\text{height}}$ 

\vsitem \xparallelfor node $\gets 0$ \xto \#leaves $-1$ \xdo
\vsitem \T leaf\_id $\gets$ (root\_id $- 1$) $\times$ \#leaves $+ $ node 
\vsitem \T \xif last stage \xthen $y$[stage\_id][leaf\_id][0] $\gets$ $a$[stage\_id][leaf\_id][0]
\vsitem \T \xelse \textsc{Compute-Output-Arrays}$(y, \text{stage\_id + 1, leaf\_id})$

\vsitem \xparallelfor $i \gets 0$ \xto $n-1$ \xdo \label{line:spawnoutputcells-fft}
\vsitem \T  \textsc{Compute-Output-Cell}($y$, stage\_id, root\_id, $i, n$, height)

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Output-Cell}(y, \text{stage\_id, node\_id, $i, n$, height})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif height $= 0$ \xthen \xreturn $a$[stage\_id + 1][node\_id][$i$]

\vsitem \xparallelfor $k \gets 0$ \xto $1$ \xdo
\vsitem \T child\_id $\gets$ (node\_id $- 1$) $\times 2 + k$
\vsitem \T $t[k] \gets 0$; coeff $\gets$ \textcolor{red}{?}
\vsitem \T new\_$i$ $\gets$  \textcolor{red}{?}
\vsitem \T $t[k] \gets$ coeff $\times$ \textsc{Compute-Output-Cell}($y$, stage\_id, child\_id, new\_$i$, $n/2$, height $- 1$)
\vsitem \xreturn $t[0] + t[1]$

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\caption{The 2-way \textsc{FFT} algorithm.}
\label{fig:fft-pseudocode-2way}
\vspace{-0.2cm}
\end{figure*}

\begin{figure*}
\begin{minipage}{\textwidth}
\begin{mycolorbox}{$\textsc{Compute-Output-Arrays}(X, \text{stage\_id, root\_id})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem treat $X$ as $\sqrt{n} \times \sqrt{n}$ matrix
\vsitem height $\gets$ \#levels in the stage; \#leaves $\gets 2^{\text{height}}$ 

\vsitem \xparallelfor node $\gets 0$ \xto \#leaves $-1$ \xdo
\vsitem \T leaf\_id $\gets$ (root\_id $- 1$) $\times$ \#leaves $+ $ node
\vsitem \T new\_$X \gets$ \textcolor{red}{?}
\vsitem \T \xif last stage \xthen $X$[stage\_id][leaf\_id][0,0] $\gets$ $a$[stage\_id][leaf\_id][0,0]
\vsitem \T \xelse \textsc{Compute-Output-Arrays}$($new\_$X, \text{stage\_id + 1, leaf\_id})$

\vsitem \xparallelfor $i \gets 0$ \xto $\sqrt{n}-1$ \xdo \label{line:spawncells-i-snfft}
\vsitem \T $X$[stage\_id][root\_id][$i,..$] $\gets$ \textsc{Compute-Output-Row}($X$[stage\_id, root\_id], stage\_id, root\_id, $i, \sqrt{n}$, height)

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\vgap{}
\begin{mycolorbox}{$\textsc{Compute-Output-Row}(Y, \text{stage\_id, root\_id, $i, n$, height})$}
\begin{minipage}{0.99\textwidth}
{\codesize
\algotopspace{}
\noindent
\begin{enumerate}
\setlength{\itemindent}{-2em}

\vsitem \xif height $= 0$ \xthen \xreturn $X$[stage\_id + 1][node\_id][$i,..$]

\vsitem \xparallelfor $j \gets 0$ \xto $\sqrt{n}-1$ \xdo
\vsitem \T child\_id $\gets$ (node\_id $- 1$) $\times \sqrt{n} + j$
\vsitem \T $y[j] \gets 0$; coeff $\gets (\omega_n)^{-ij}$
\vsitem \T new\_$X \gets$ \textcolor{red}{?}; new\_$i$ $\gets$  \textcolor{red}{?}
\vsitem \T $y[j] \gets$ coeff $\times$ \textsc{Compute-Output-Row}(new\_$X$, stage\_id, child\_id, new\_$i$, $\sqrt{n}$, height $- 1$) \vsitem \xreturn \textsc{Compute-Output-Row}($y$, stage\_id, child\_id, $i$, $\sqrt{n}$, height $- 1$)

\algobottomspace{}
\end{enumerate}
}
\end{minipage}
\end{mycolorbox}
\end{minipage}
\caption{The $\sqrt{n}$-way \textsc{FFT} algorithm.}
\label{fig:fft-pseudocode-sqrtnway}
\vspace{-0.2cm}
\end{figure*}

\hide{
\begin{lemma}
\label{lem:computing-output-array}
The complexity of \textsc{Compute-Output-Arrays} is $T_1(n) = \Oh{n \psi \log n / \log \psi}$, $T_{\infty}(n) = \Oh{\log^2 n / \log \psi}$, and $S_{\infty}(n) = \Oh{n \log n / \log \psi}$.
\end{lemma}
\begin{proof} $[$Work.$]$ We compute the output matrix in $h+1$ \bands $S_0, S_1, \ldots, S_{h}$, where $h = \log n / \log \psi$. Suppose $W_i$ defines the work done at \band $S_i$. We first come up with a generic formula for $W_i$. We use a direct proof to show that $W_i = \Oh{n \psi}$, which implies that the total work is $\sum_{i = 0}^{h} W_i = \Oh{n \psi \log n / \log \psi}$.

We compute $W_i$ for $i \in [0, h]$. Each output array at the root level of stage $S_i$ is constructed from the output arrays at the leaf level of the stage. All cells in all output arrays at the root level of stage $S_i$ are computed in parallel. \#Nodes at the root level of \band $S_i$ is $2^{i\log \psi} = \psi^i$. Each such array has $n/2^{i \log \psi} = n / \psi^i$ cells. Each cell at a recursion level $\ell$ depends on exactly $2$ output cells in recursion level $\ell +1$. Hence, each cell in the array at the root level of stage $S_i$ depends on $\mathcal{O}(2^{\log \psi}) = \Oh{\psi}$ cells in an array at the leaf level of the stage. Hence, $W_i = \Oh{n \psi}$ for all $i \in [0, h]$. Combining the work of all \bands, we get $T_1(n) = \sum_{i = 0}^{h} W_i = \Oh{n \psi \log n / \log \psi}$.

\vspace{0.1cm}
\noindent
[Span.] Let $T_{\infty}(m, i)$ denote the span of the \textsc{Compute-Output-Arrays} algorithm starting from stage $i$ where an array at the root level is of size $m$. We give a recursive formula to compute $T_{\infty}(m, i)$. Then, the total span for the algorithm is $T_{\infty}(n, 0)$.

Consider the \textsc{Compute-Output-Arrays} algorithm.
\#Nodes at the leaf level of stage $S_i$ is $\psi^i$. Launching these nodes in parallel incurs a span of $\Oh{i \log \psi}$. An array at the leaf level will be of size $m/2^{\log \psi} = m / \psi$. Spawning \textsc{Compute-Output-Cell} function for all cells (line \ref{line:spawnoutputcells-fft}) incurs a span of $\Oh{i \log \psi + \log (m/\psi)}$. Executing the \textsc{Compute-Output-Cell} algorithm incurs $\Oh{\log \psi}$ span. Adding all these spans give us $\Oh{i \log \psi + \log m} = \Oh{\log (m\psi^i)}$.

The span of stage $S_i$ recursively depends upon the span of stage $S_{i + 1}$ as the output arrays at the leaf level of stage $S_{i + 1}$ are constructed from the leaf level arrays of stage $S_{i}$. Hence, $T_{\infty}(m,i)$ can be recursively defined using the previous analysis as:
$T_{\infty}(m,i) = \Oh{\log \psi}$ if $i = h$ and $T_{\infty}(m,i) = \Oh{\log (m\psi^i)} + T_{\infty}(m/\psi,i+1)$ if $i < h$.

By unrolling the recursion and simplifying, we compute the total span as $T_{\infty}(n,0) = \Oh{\log^2 n / \log \psi}$.\\
 
\vspace{-0.2cm}
\noindent
[Space.] The space requirement at each stage is $\Oh{n}$ and there are $\log n / \log \psi$ stages. Hence, the total space is $\Oh{n \log n / \log \psi}$.
\end{proof}
}















\begin{lemma}
\label{lem:computing-output-array}
The complexity of \textsc{Compute-Output-Arrays} is $T_1(n) = \Oh{n \psi \log n / \log \psi}$, $T_{\infty}(n) = \Oh{\log^2 n / \log \psi}$, and $S_{\infty}(n) = \Oh{n \log n / \log \psi}$.
\end{lemma}
\begin{proof} $[$Work.$]$ We compute the output matrix in $h+1$ \bands $S_0, S_1, \ldots, S_{h}$, where $h = \log n / \log \psi$. Suppose $W_i$ defines the work done at \band $S_i$. We first come up with a generic formula for $W_i$. We use a direct proof to show that $W_i = \Oh{n \psi}$, which implies that the total work is $\sum_{i = 0}^{h} W_i = \Oh{n \psi \log n / \log \psi}$.

We compute $W_i$ for $i \in [0, h]$. Each output array at the root level of stage $S_i$ is constructed from the output arrays at the leaf level of the stage. All cells in all output arrays at the root level of stage $S_i$ are computed in parallel. \#Nodes at the root level of \band $S_i$ is $2^{i\log \psi} = \psi^i$. Each such array has $n/2^{i \log \psi} = n / \psi^i$ cells. Each cell at a recursion level $\ell$ depends on exactly $2$ output cells in recursion level $\ell +1$. Hence, each cell in the array at the root level of stage $S_i$ depends on $\mathcal{O}(2^{\log \psi}) = \Oh{\psi}$ cells in an array at the leaf level of the stage. Hence, $W_i = \Oh{n \psi}$ for all $i \in [0, h]$. Combining the work of all \bands, we get $T_1(n) = \sum_{i = 0}^{h} W_i = \Oh{n \psi \log n / \log \psi}$.

\vspace{0.1cm}
\noindent
[Span.] Let $T_{\infty}(m, i)$ denote the span of the \textsc{Compute-Output-Arrays} algorithm starting from stage $i$ where an array at the root level is of size $m$. We give a recursive formula to compute $T_{\infty}(m, i)$. Then, the total span for the algorithm is $T_{\infty}(n, 0)$.

Consider the \textsc{Compute-Output-Arrays} algorithm.
\#Nodes at the leaf level of stage $S_i$ is $\psi^i$. Launching these nodes in parallel incurs a span of $\Oh{i \log \psi}$. An array at the leaf level will be of size $m/2^{\log \psi} = m / \psi$. Spawning \textsc{Compute-Output-Cell} function for all cells (line \ref{line:spawnoutputcells-fft}) incurs a span of $\Oh{i \log \psi + \log (m/\psi)}$. Executing the \textsc{Compute-Output-Cell} algorithm incurs $\Oh{\log \psi}$ span. Adding all these spans give us $\Oh{i \log \psi + \log m} = \Oh{\log (m\psi^i)}$.

The span of stage $S_i$ recursively depends upon the span of stage $S_{i + 1}$ as the output arrays at the leaf level of stage $S_{i + 1}$ are constructed from the leaf level arrays of stage $S_{i}$. Hence, $T_{\infty}(m,i)$ can be recursively defined using the previous analysis as:
$T_{\infty}(m,i) = \Oh{\log \psi}$ if $i = h$ and $T_{\infty}(m,i) = \Oh{\log (m\psi^i)} + T_{\infty}(m/\psi,i+1)$ if $i < h$.

By unrolling the recursion and simplifying, we compute the total span as $T_{\infty}(n,0) = \Oh{\log^2 n / \log \psi}$.\\
 
\vspace{-0.2cm}
\noindent
[Space.] The space requirement at each stage is $\Oh{n}$ and there are $\log n / \log \psi$ stages. Hence, the total space is $\Oh{n \log n / \log \psi}$.
\end{proof}

==> mmtc-litreview.tex <==
\section{Background}

Cache efficiency depends heavily on the data structure in use; exploring the options in this area, \cite{bially1969space} presented a set of self-similar space filling curves which can be efficiently generated by finite state machine based algorithms. Later, Wise et al. \cite{wise2000ahnentafel} gave a matrix ordering scheme that preserves data locality while allowing quad tree representation (an extension of Morton ordering).

Although Strassen's algorithm \cite{Strassen1969} for matrix multiplication takes less than $4.7 n^{2.8}$ operations, it was meant to minimize work, not cache efficiency. In practice iterative and recursive schemes that have worse RAM complexity (but better cache complexity) are generally used - some empirical comparisons are given in \cite{thottethodi1998tuning}, as well as a new algorithm for managing bandwidth while performing MM.

Tight upper and lower bounds on the number of I/O operations required by algorithms closely related to MM (including matrix transposition and FFT) are given in \cite{aggarwal1988input}. Frigo et al. \cite{frigo2012cache} provided baseline work on cache oblivious algorithms, including analysis of the cache complexity of iterative MM compared with Strassen's algorithm. They also analyze a veriety of other algorithms' cache ecomplexity, including FFT, matrix transposition, funnlesort, and distributionsort.

In classical distributed-memory matrix multiplication algorithms, known as $2D$ algorithms, only one copy of each input/output matrix is distributed across all $p$ processors of a $\sqrt{p} \times \sqrt{p}$ processor grid \cite{cannon1969cellular}. These algorithms have $\Th{{n^2}/{\sqrt{p}}}$ bandwidth and $\Th{\sqrt{p}}$ latency, and they balance the load \cite{irony2004communication, ballard2011minimizing, ballard2014communication}.

Another class of distributed-memory matrix multiplication algorithms, called $3D$ algorithms, distribute $p^\frac{1}{3}$ copies of the input matrix across a $3D$ processor grid of size $p^\frac{1}{3} \times p^\frac{1}{3} \times p^\frac{1}{3}$ \cite{dekel1981parallel,agarwal1995three,aggarwal1990communication,johnsson1993minimizing}. It has been shown \cite{irony2004communication,ballard2011minimizing} that in addition to balancing load these algorithms minimize communication, with $\Th{\log(p)}$ latency and $\Th{{n^2}/{p^\frac{2}{3}}}$ bandwidth \cite{solomonik2011communication}. The final class of matrix multiplication algorithms interpolate between the $2D$ and $3D$ algorithms in the sense that they distribute $c \in \{1, 2, ..., p^{{1}/{3}}\}$ copies of the input matrix across a processor grid of size $({p}/{c})^{{1}/{2}} \times ({p}/{c})^{{1}/{2}} \times c$ and hence, they are called $2.5D$. These algorithms have $\Th{{n^2}/{\sqrt{cp}}}$ bandwidth and $\Oh{ \sqrt{{p}/{c^3}} + \log(c) }$ latency. The interpolation technique can be used for Gaussian-elimination style LU decomposition algorithm to obtain $\Th{{n^2}/{\sqrt{cp}}}$ bandwidth and $\Oh{\sqrt{cp} \log{p}}$ latency which are asymptotically optimal for any choice of $c$ (modulo $\log(p)$ factor for latency). Ballard., et al \cite{ballard2012communication} have proved that Communication-Avoiding Parallel Strassen (CAPS) meets the bandwidth and latency lower bounds on distributed-memory parallel machines.

Tensor is a generalization of multidimensional matrix which is widely used in many scientific disciplines \cite{Kolda2009, Coppi2009, Smilde2004, Vasilescu2002, Abadi16, Vasilache2014, Harrison2016, Frigo2005}.

Naive Dense Tensor Contraction involves writing explicit loop-based implementation which is equivalent to triply nested loop implementation of 2D matrix-multiplication. Loop based implementation has very poor cache complexity hence poor real time performance. Apra et al. and Bibireata et al. have tried optimizing Tensor Contraction by loop transformations to improve over the naive loop based implementation \cite{Apra2014, Bibireata2003}. While the downside of these improvements is that it suffers from suboptimal strided memory access, Stock et al. and Harrison et al. explored vectorizing the loop-based tensor contraction for small tensors \cite{Stock2011, Harrison2004}. Ma et al. and Nelson et al. separately developed high-performance code generators for GPUs \cite{Ma2011, Nelson2015} for looping based Tensor Contraction. 

In order to avoid the sub-optimal memory access and memory transfer for higher dimensional tensor, researchers converted the higher dimensional tensor into matrix via flattening and transposition to cast a single GEMM and transposing the resulting matrix back to the desired shape of tensor. Transpose-Transpose-GEMM-Transpose (TTGT) based tool TCE \cite{Hirata2003} exploits the highly efficient GEMM kernel implementations such as optimized BLAS Libraries \cite{Whaley2005}, Intel’s Math Kernel Library \cite{mkl2003} etc. by converting tensors to matrix like kernels. Potential problems of this approach is that it requires additional memory during transposition and introduces pure overhead of pre- and post-processing step. In many cases this overhead dominates the runtime and becomes infeasible to the bandwidth-bound computation environments. 

Napoli et al. and Li et al. devised a technique of slicing the tensors into a series of small 2D tensors and contract them via GEMM \cite{DiNapoli2014, Li2015}. This works well when all the tensors are of huge size. The performance depends on the size of the slices hence the initial tensor shape.  Springer et al. developed A high-performance compiler for tensor transpositions \cite{ttc2016a} to minimize the pre- and post-processing overhead of tensor transposition. GEMM-like Tensor-Tensor multiplication (GETT) \cite{Springer2018} exploits the CPU’s cache hierarchy, avoids explicit preprocessing steps, and operates on arbitrary dimensional sub-tensors while preserving stride-one memory accesses to achieve high-performance implementation. GETT prepares sub-blocks of tensors to fit in the CPU cache and fuses the transposition operation with the GEMM computations. Devin Matthews independently developed TBLIS \cite{Matthews2018} which shares the same idea of GETT but it supports all forms of tensor contractions including which cannot be mapped to GEMM like kernels. 

Shi et al. \cite{shi2016tensor} have proposed and evaluated new BLAS-like primitives that are capable of performing a wide range of tensor contractions on CPU and GPU effectively without any explicit memory motion. They have summarized existing approaches and present library-based approaches that avoid memory movement. They have obtained a significant speedup (10x on GPU and 2x on CPU) for small and moderate tensor sizes. Their approach is effective for applications where tensor sizes tend to be small, but required numerous tensor contraction operations to be performed successively. Recently, Kim et al. \cite{kim2019code} have proposed a high-performance GPU code generator for arbitrary tensor contractions. For effective code generation scheme, the proposed framework exploits the domain-specific properties of the data reuse in the tensor computation. Their framework uses an effective model-driven search to determine the parameters for mapping the computation to threads and staging of data through the GPU memory hierarchy.

Solomonik et al. \cite{solomonik2012preliminary, solomonik2014massively, solomonik2013cyclops} have designed a framework called Cyclops (cyclic-operations) Tensor Framework (CTF). Using massively-parallel supercomputers, this framework can scale high-dimensional tensor contractions in Coupled Cluster calculations. CTF employs a cyclic distribution to preserve symmetry in subtensors with minimum required padding. This leads to a completely regular decomposition of tensors capable of applying classic linear algebra optimizations. The framework executes a completely load balanced symmetry-preserving algorithm for tensor contractions. They have proved that their framework meets the lower bound of communication cost with minimal padding required. Achieving the lower bound of communication is obtained due to the fact that CTF minimizes the storage demands on the memory by considering symmetry in the tensors of Coupled Cluster calculations. Preserving symmetry in sub-tensors of a tensor enforces the decomposition to use the same cyclic phase among symmetric decomposition of that tensor. However, in order to have a flexibility of mapping onto any physical topology, CTF uses an efficient virtualized mapping of the tensors, which overdecomposes the tensors and then maps the blocks onto the processor grid. Applying multiple tensor contractions one after another can restrict the mapping of the tensors to the processors. CTF has implemented highly optimized tensor redistribution kernels. For the three class of algorithms (Nonsymmetric Contraction Algorithm, Direct Evaluation Algorithm and Symmetry Preserving Tensor Contraction Algorithm), Solomonik et al. \cite{solomonik2015communication,solomonik2014massively} have also provided the sequential and parallel lower bounds of communication cost and discussed the attainability of the bounds. They have also explored the potential of using 2D, 3D, and 2.5D processor grid with communication cost analysis.

For a wide class of quantum chemistry computations, several researchers \cite{baumgartnercompile, baumgartner2005synthesis, ma2011practical} have provided program synthesis systems and tools, including CTF, RRR, and CAST which apply several compile-time optimizations based on analytical performance model to the given tensor contraction expression. Optimizations are memory usage minimization, space-time transformation, communication minimization, data distribution and task partitioning among the parallel processors, and data locality optimization. For TCE, Gao et al. \cite{gao2005performance} have introduced a performance model for measuring the disk I/O as well as inter-processor communication cost. Kjolstad et al. \cite{kjolstad2017taco} have developed taco, a code generation tool that produces dense, sparse, and mixed kernels from tensor algebra expressions. Additionally, \cite{susungi2017towards} have proposed an easily extensible intermediate language to express tensor computations and code transformations in a modular and generative fashion.


\cite{prokop1999cache} presented early work on the \emph{tall cache model} (a tall cache is one where the total cache size $Z$ is of order $\Omega(L^2)$, with block size $L$), emphazising the importance of cache obliviousness and carrying out full analyses of the cache complexity of a few common matrix multiplication algorithms under various data ordering schemes. They compare the tall cache model to two-level models memory heirachies \cite{aggarwal1988input, vitter1994algorithms}.

A set of algorithms that are optimal in terms of I/O operations for matrix multiplications were given in \cite{vitter1994algorithms}, which uses the two-level memory model for the first time. The two-level memory model was designed to produce a more accurate description of parallel block transfer (each of $P$ secondary storage devices can simultaneously transfer a block). Note: The focus in \cite{vitter1994algorithms} is on algorithms for distributed computing systems, not shared memory systems.

The heirarchical memory model (HMM) was presented in \cite{aggarwal1987model}, which assumes that accessing data stored in register $x$ takes $\lceil \log x \rceil$ time, and that the register $x$ has $2^x$ blocks. Subsequent developments were presented in \cite{alpern1994uniform} with the uniform memory heirarchy (UMH) model, as well as the metric of \emph{communication efficiency}: the fraction of time during which the processor is active, rather than waiting for memory to transfer. Some empirically optimized UMH-efficient programs for matrix transposition and multiplication as well as FFT were given. The UMH model was intended for (single core) shared memory devices, but a possible generalization for distributed computing applications was included.

An empirical analysis of the performance of MM on GPUs is given in \cite{fatahalian2004understanding}. GPU-based MM implementations are not (in general) as good as cache aware CPU approaches because of a data bandwidth bottleneck; see \cite{thottethodi1998tuning, whaley2001automated}. \cite{fatahalian2004understanding} also provides benchmark data showing that cache efficient CPU algorithms can be as fast or faster than GPU based MM algorithms.

Some recursive memory layouts are discussed in \cite{chatterjee2002recursive}, which compares recursion depth vs performance on different matrix multiplication algorithms (specifically: the cannonical algorithms, Strassen's algorithm, and the Winograd variant of Strassen's algorithm). Emphasis is placed on the complexity of computing addresses for given matrix elements, and in achieving \emph{memory locality} - it is best to use data which is contiguous in memory. Complexity of the data structure is mentioned as an easily overlooked sink of computation: perhaps a given ordering seems more efficient because it shifts computation into the addresses of matrix elements, which are then ignored in the analysis. \cite{chatterjee2002recursive} also makes the point that selection of the data structure recursion cutoff point is important - standard ordering is best once data blocks can fit into cache.

\cite{lam1991cache} is an important study on how performance changes as a function of cache block sizes used for matrix storage. They provides a very comprehensive analysis, and show spacial locality to be preferable when it is possible to achieve. They also suggest a set of heuristics for use in designing cache aware algorithms (e.g. block size should be small \emph{with respect to cache size}, and to a lesser extent dependent on matrix size).

\cite{yzelman2009cache} analyzes a cache oblivious algorithm for spare matrix multiplication, and presents a new ordering method (zig-zag CRS) as well as a new approach to SpMV (sparse matrix-vector multiplication) based on hypergraph partitioning. Experimental results are included.



